LiDARTag: A Real-Time Fiducial Tag System for Point Clouds

Image-based fiducial markers are useful in problems such as object tracking in cluttered or textureless environments, camera (and multi-sensor) calibration tasks, and vision-based simultaneous localization and mapping (SLAM). The state-of-the-art fiducial marker detection algorithms rely on the consistency of the ambient lighting. This paper introduces LiDARTag, a novel fiducial tag design and detection algorithm suitable for light detection and ranging (LiDAR) point clouds. The proposed method runs in real-time and can process data at 100 Hz, which is faster than the currently available LiDAR sensor frequencies. Because of the LiDAR sensors' nature, rapidly changing ambient lighting will not affect the detection of a LiDARTag; hence, the proposed fiducial marker can operate in a completely dark environment. In addition, the LiDARTag nicely complements and is compatible with existing visual fiducial markers, such as AprilTags, allowing for efficient multi-sensor fusion and calibration tasks. We further propose a concept of minimizing a fitting error between a point cloud and the marker's template to estimate the marker's pose. The proposed method achieves millimeter error in translation and a few degrees in rotation. Due to LiDAR returns' sparsity, the point cloud is lifted to a continuous function in a reproducing kernel Hilbert space where the inner product can be used to determine a marker's ID. The experimental results, verified by a motion capture system, confirm that the proposed method can reliably provide a tag's pose and unique ID code. The rejection of false positives is validated on the Google Cartographer indoor dataset and the Honda H3D outdoor dataset. All implementations are coded in C++ and are available at: https://github.com/UMich-BipedLab/LiDARTag.

==> Calibration.tex <==
\section{Calibration Formulation}
\label{sec:calibration}
\bh{Modifying on progress (heading to the class)}
\mgj{The choice of estimation algorithms is confusing and not justified at all. I would argue since all measurements are SE(3), you can use SE-Sync to find the globally optimal solution. This is simply writing a \texttt{data.g2o} file and using SE-Sync library: \href{https://github.com/david-m-rosen/SE-Sync}{https://github.com/david-m-rosen/SE-Sync}}

One very important application of the LiDARTag is LiDAR-camera calibration since the tag 
can be seen from both LiDARs and cameras. If the tag is seen from a LiDAR, it is a LiDARTag 
and if it is seen from a camera, then it is an AprilTag. Since all measurements are $\SE(3)$,
we use sample mean in Lie Group.

The problem is to find a rigid body transformation between a LiDAR and a camera. The
problem then can be solved directly 3D special Euclidean group, denoted by
\begin{equation}
    \SE(3) = \left\{H = \begin{bmatrix} R & T \\ \zeros[1 \times 3] & 1\end{bmatrix}\in
    \GL_4(\realnumbers),\ | R\in\SO(3),\ T\in\realnumbers^3\right\}
\end{equation}

\subsection{State Representation}
As with typical LiDAR-camera calibration, we wish to estimate the relative orientation and
relative translation between a LiDAR and a camera. These states are represented by $R_{CL}$
and $T_{CL}$, respectively. These collection of state variables forms a matrix Lie
group, $\mathcal{G}$ and the state $X_t$ we wish to estimate:
\begin{align}
    X_t = \begin{bmatrix} R_{CL} & T_{CL} \\ \zeros[1\times 3] & 1\end{bmatrix}.
\end{align}

The measurements $\hat{H}$ can be represented by the following matrix:
\begin{align}
    H_{TL} &= \tilde{H}_{TL}\Exp(\xi_{TL}), \ \Ncal(\zeros, \Sigma_{TL}) \label{eq:H_TL}\\
    H_{TC} &= \tilde{H}_{TC}\Exp(\xi_{TC}), \ \Ncal(\zeros, \Sigma_{TC})\label{eq:H_TC}\\
    H_{CL} &= \tilde{H}_{CL}\Exp(\xi_{CL}) = H^{-1}_{TL}H_{TL}\label{eq:H_CL}\\
    \H[1:t] &= \begin{bmatrix}  H^{t=1}_{CL} & \cdots & H^{t=t}_{CL} \end{bmatrix}^\transpose\label{eq:H_acc}
\end{align}
where $H_{TL}, H_{TC}, H_{CL}$ are true rigid body transform of tag-to-LiDAR, tag-to-camera,
camera-to-LiDAR, respectively and $\H[1:t]$ is a collection of measurement until $t$.
As derived in~\citep{hartley2018contact} and~\citep{barrau2015non}, the linearization matrix $\O[1:t]$, 
innovation $\Z[1:t]$ and noise model $\N[1:t]$ are denoted by: 
\begin{align}
    \O[1:t] &= \begin{bmatrix} -\I[6,6] & \cdots & -\I[6,6]\end{bmatrix}^\transpose\\
    \Z[1:t] &= \begin{bmatrix} \Log(X_1(H^{t=1}_{CL})^{-1}) & \cdots & \Log(X_t(H^{t=t}_{CL})^{-1})\end{bmatrix}^\transpose\\
    \N[1:t] &= \diag(N_1, \cdots, N_t)
\end{align}
where $N_i = \Adjoint(X_i^{-1})N\Adjoint(X_i^{-1})^{-1}$. The full state and covariance update
equation equations of the Right-Invariant Extended Kalman Filter (RI-EKF) can be
written as:
\begin{align}
    \hat{X}_t &= X_t\Exp\left(K_t\Z[1:t] \right) \label{eq:correction_x}\\
    \hat{P}_t &= (\I[6,6]-K_t\O[1:t])P_t \label{eq:correction_P}
\end{align}
where the gain $K_t$ is computed using 
\begin{align}
    S_t &= \O[1:t]P_t\O[1:t][\transpose] + \N[1:t]\\
    K_t &= P_t\O[1:t][\transpose]S_t^{-1}
\end{align}

If we have the truth transformation $X_{\text{truth}}$, the error $e$ of the calibration 
can be written as follow:
\begin{align}
    e = \lVert \Log(X_{\text{truth}}\hat{X}_t^{-1}) \rVert_2
    \label{eq:calibration_acc}
\end{align}

\subsubsection{Bias estimation}
\label{sec:bias}
Given a measured LiDARTag pose, $\tilde{H}_{TL}$ and a measured AprilTag pose, $\tilde{H}_{TC}$, 

\label{sec:calibration_formulation}

% \begin{figure}[t]%
% \centering
% \subfigure[][Frame definitions of a camera, lidar and a tag.]{%
% \label{fig:frame}%
% \includegraphics[width=0.45\columnwidth]{frame.png}}%
% \hspace{8pt}%
% \subfigure[][\red{CHANGE}]{%
% % \label{fig:tag_explain}%
% \includegraphics[width=0.45\columnwidth]{tag_explain.png}}%
% \caption[]{\red{FILLIN}}%
% \label{fig:calibration}%
% \end{figure}

\begin{figure}[t]%
\centering
\includegraphics[width=0.5\columnwidth]{frame.png}%
\caption[]{Frame definitions of a camera, a LiDAR and a tag. If the tag is observed by the camera, it is an AprilTag. On the other hand, if it is observed by the LiDAR, it is a LiDARTag. $\hat{H}_{TC}$ is the pose measurement between the camera and the AprilTag. $\hat{H}_{TL}$ is the pose measurement between the LiDAR and the LiDARTag. We estimate a rigid body transformation between the LiDAR and the camera, $\hat{H}_{CL}$, as the calibration parameter. \mgj{The two-sided red arrow doesn't make sense. Make it one-sided. One side is the inverse of the other side so it can't represent both.}}%

\label{fig:frame}%
% \label{fig:calibration}%
\end{figure}

\subsection{Sample Mean}
% From \eqref{eq:H_acc}, the mean $\hat{X}_{\text{mean}}$ is simply:
% \begin{align}
%     \hat{X}_{\text{mean}} &= \Exp(\frac{\sum_{i=1}^t(\Log(H_{CL}^{t=i}))}{t}),
% \end{align}
% and error $e$ is the same as \eqref{eq:calibration_acc} but with $\hat{X}_t = \hat{X}_{\text{mean}}$.

Given a matrix Lie group $\mathcal{G}$ and a set of t samples $H_{CL}^{i}\in\mathcal{G},$
we can estimate the mean and covariance iteratively as follow~\citep{eade2013lie}:
\begin{align}
    \nu_{i,k} &\coloneqq\Log\left(H_{CL}^{t=i}X_k^{-1}\right)\\
    \Sigma_k &= \frac{1}{t}\sum_{i=1}^{t}\nu_{i,k}\nu_{i,k}^\transpose\\
    X_{k+1} &= \Exp(\frac{1}{t}\sum_{i=1}^{i=t}\nu_{i,k})X_k
\end{align}
Since any of the samples provides an initial guess for the mean $X_0$, without loss of
generality, we can assume $X_0 = H_{CL}^{t=0}$. It usually converges in a few
iterations (less than 10).



==> Calibration_.tex <==
\section{Calibration Formulation}
\label{sec:calibration}
\bh{Modifying on progress (heading to the class)}
\mgj{The choice of estimation algorithms is confusing and not justified at all. I would argue since all measurements are SE(3), you can use SE-Sync to find the globally optimal solution. This is simply writing a \texttt{data.g2o} file and using SE-Sync library: \href{https://github.com/david-m-rosen/SE-Sync}{https://github.com/david-m-rosen/SE-Sync}}

One very important application of the LiDARTag is LiDAR-camera calibration since the tag 
can be seen from both LiDARs and cameras. If the tag is seen from a LiDAR, it is a LiDARTag 
and if it is seen from a camera, then it is an AprilTag. We compare results of the three methods
in $\SE(3)$: average mean, sampling mean and the Invariant Extended Kalman Filtering 
(InEKF)~\cite{hartley2018contact}~\cite{barrau2015non}~\cite{barrau2016invariant}~\cite{barrau2018invariant}.

The problem is to find a rigid body transformation between a LiDAR and a camera. The
problem then can be solved directly 3D special Euclidean group, denoted by
\begin{equation}
    \SE(3) = \left\{H = \begin{bmatrix} R & T \\ \zeros[1 \times 3] & 1\end{bmatrix}\in
    \GL_4(\realnumbers),\ | R\in\SO(3),\ T\in\realnumbers^3\right\}
\end{equation}


\subsection{Invariant Extended Kalman Filtering}
Since all the measurement and state are in $\SE(3)$, the InEKF technique can also be used to 
estimate the homogeneous transformation. Additionally, InEKF has characteristic of fast 
convergence even with bad initialization.
In order to be consistent with the standard InEKF theory, the biases are neglected for now and 
will be addressed in in Sec. \ref{sec:bias}.

\subsubsection{State Representation}
As with typical LiDAR-camera calibration, we wish to estimate the relative orientation and
relative translation between a LiDAR and a camera. These states are represented by $R_{CL}$
and $T_{CL}$, respectively. These collection of state variables forms a matrix Lie
group, $\mathcal{G}$ and the state $X_t$ and the noise $N$ can be represented by the following matrix:
\begin{align}
    X_t = \begin{bmatrix} R_{CL} & T_{CL} \\ \zeros[1\times 3] & 1\end{bmatrix}, \ \
    N = \diag(\epsilon_{3,3}, \delta_{3,3},)
\end{align}
where $\epsilon$ and $\delta$ are rotation noise and translation noise, respectively.

Since the LiDAR and the camera are static, the motion model $u_t$ is an Identity
matrix \mgj{motion model $u_t$? Don't introduce new variables and math if it's not necessary.}. The measurement are modeled in right invariant error as being corrupted by
additive white Gaussian noise \mgj{How do you get/set the noise covariances? How sensitive are they? This needs to be explained clearly, if the noise model for measurements is used.}:
\begin{align}
    H_{TL} &= \tilde{H}_{TL}\Exp(\xi_{TL}), \ \Ncal(\zeros, \Sigma_{TL}) \label{eq:H_TL}\\
    H_{TC} &= \tilde{H}_{TC}\Exp(\xi_{TC}), \ \Ncal(\zeros, \Sigma_{TC})\label{eq:H_TC}\\
    H_{CL} &= \tilde{H}_{CL}\Exp(\xi_{CL}) = H^{-1}_{TL}H_{TL}\label{eq:H_CL}\\
    \H[1:t] &= \begin{bmatrix}  H^{t=1}_{CL} & \cdots & H^{t=t}_{CL} \end{bmatrix}^\transpose\label{eq:H_acc}
\end{align}
where $H_{TL}, H_{TC}, H_{CL}$ are true rigid body transform of tag-to-LiDAR, tag-to-camera,
camera-to-LiDAR, respectively and $\H[1:t]$ is a collection of measurement until $t$.
As derived in~\cite{hartley2018contact} and~\cite{barrau2015non}, the linearization matrix $\O[1:t]$, 
innovation $\Z[1:t]$ and noise model $\N[1:t]$ are denoted by: 
\begin{align}
    \O[1:t] &= \begin{bmatrix} -\I[6,6] & \cdots & -\I[6,6]\end{bmatrix}^\transpose\\
    \Z[1:t] &= \begin{bmatrix} \Log(X_1(H^{t=1}_{CL})^{-1}) & \cdots & \Log(X_t(H^{t=t}_{CL})^{-1})\end{bmatrix}^\transpose\\
    \N[1:t] &= \diag(N_1, \cdots, N_t)
\end{align}
where $N_i = \Adjoint(X_i^{-1})N\Adjoint(X_i^{-1})^{-1}$. The full state and covariance update
equation equations of the Right-Invariant Extended Kalman Filter (RI-EKF) can be
written as:
\begin{align}
    \hat{X}_t &= X_t\Exp\left(K_t\Z[1:t] \right) \label{eq:correction_x}\\
    \hat{P}_t &= (\I[6,6]-K_t\O[1:t])P_t \label{eq:correction_P}
\end{align}
where the gain $K_t$ is computed using 
\begin{align}
    S_t &= \O[1:t]P_t\O[1:t][\transpose] + \N[1:t]\\
    K_t &= P_t\O[1:t][\transpose]S_t^{-1}
\end{align}

If we have the truth transformation $X_{\text{truth}}$, the error $e$ of the calibration 
can be written as follow:
\begin{align}
    e = \lVert \Log(X_{\text{truth}}\hat{X}_t^{-1}) \rVert_2
    \label{eq:calibration_acc}
\end{align}

\subsubsection{Bias estimation}
\label{sec:bias}
Given a measured LiDARTag pose, $\tilde{H}_{TL}$ and a measured AprilTag pose, $\tilde{H}_{TC}$, 

\label{sec:calibration_formulation}

% \begin{figure}[t]%
% \centering
% \subfigure[][Frame definitions of a camera, lidar and a tag.]{%
% \label{fig:frame}%
% \includegraphics[width=0.45\columnwidth]{frame.png}}%
% \hspace{8pt}%
% \subfigure[][\red{CHANGE}]{%
% % \label{fig:tag_explain}%
% \includegraphics[width=0.45\columnwidth]{tag_explain.png}}%
% \caption[]{\red{FILLIN}}%
% \label{fig:calibration}%
% \end{figure}

\begin{figure}[t]%
\centering
\includegraphics[width=0.5\columnwidth]{frame.png}%
\caption[]{Frame definitions of a camera, a LiDAR and a tag. If the tag is observed by the camera, it is an AprilTag. On the other hand, if it is observed by the LiDAR, it is a LiDARTag. $\hat{H}_{TC}$ is the pose measurement between the camera and the AprilTag. $\hat{H}_{TL}$ is the pose measurement between the LiDAR and the LiDARTag. We estimate a rigid body transformation between the LiDAR and the camera, $\hat{H}_{CL}$, as the calibration parameter. \mgj{The two-sided red arrow doesn't make sense. Make it one-sided. One side is the inverse of the other side so it can't represent both.}}%

\label{fig:frame}%
% \label{fig:calibration}%
\end{figure}

\subsection{Sample Mean}
% From \eqref{eq:H_acc}, the mean $\hat{X}_{\text{mean}}$ is simply:
% \begin{align}
%     \hat{X}_{\text{mean}} &= \Exp(\frac{\sum_{i=1}^t(\Log(H_{CL}^{t=i}))}{t}),
% \end{align}
% and error $e$ is the same as \eqref{eq:calibration_acc} but with $\hat{X}_t = \hat{X}_{\text{mean}}$.

Given a matrix Lie group $\mathcal{G}$ and a set of t samples $H_{CL}^{i}\in\mathcal{G},$
we can estimate the mean and covariance iteratively as follow~\cite{eade2013lie}:
\begin{align}
    \nu_{i,k} &\coloneqq\Log\left(H_{CL}^{t=i}X_k^{-1}\right)\\
    \Sigma_k &= \frac{1}{t}\sum_{i=1}^{t}\nu_{i,k}\nu_{i,k}^\transpose\\
    X_{k+1} &= \Exp(\frac{1}{t}\sum_{i=1}^{i=t}\nu_{i,k})X_k
\end{align}
Since any of the samples provides an initial guess for the mean $X_0$, without loss of
generality, we can assume $X_0 = H_{CL}^{t=0}$. It usually converges in a few
iterations (less than 10).



==> DetectorShort.tex <==
\begin{figure*}[t!]%
\centering
\subfloat[]{%
\label{fig:edges}%
\includegraphics[height=0.18\textwidth]{GroupedFeatures.png}}~
\hspace{2pt}%
\subfloat[]{%
\label{fig:filled}%
\includegraphics[height=0.18\textwidth]{FilledCluster.png}}~
\hspace{2pt}%
\subfloat[]{%
\label{fig:boundary}%
\includegraphics[height=0.18\textwidth]{BoundaryPionts.png}}~
\hspace{2pt}%
\subfloat[]{%
\label{fig:PlanarTemplate}%
\includegraphics[height=0.18\textwidth]{PlanerTemplate.png}}~
\hspace{2pt}%
\subfloat[]{%
\label{fig:3DTemplate}%
\includegraphics[height=0.18\textwidth]{Front3DShape.png}}~
\hspace{2pt}%
\subfloat[]{%
\label{fig:3DTamplateSide}%
\includegraphics[height=0.18\textwidth]{Side3DShape.png}}
\caption[]{
    Intermediate steps of the LiDARTag system. The system takes a full scan
point cloud and applies feature detection as defined in 
\eqref{eq:GD} and associates the features into clusters (magenta spheres), as shown
in~\subref{fig:edges}. Using the features, the clusters are filled from the
original scan (different color dots stand for different intensity values) as shown
in~\subref{fig:filled}. Later, boundary points (indicated by boxes) are detected.
After validating all the clusters, \subref{fig:PlanarTemplate} shows the result of
the point cloud of a \lidart
pulled back to the \lidar origin by $H_T^L$, which is a rigid-body
transformation from the tag to the \lidar that minimizes an $L_1$-inspired fitting
error \eqref{eq:JKHcost}. The green box is the template of the fiducial marker.
\subref{fig:3DTemplate} and \subref{fig:3DTamplateSide} describe the side front view
and the side view of a 3D-shape point cloud constructed based on the intensity of the
pullback point cloud. This 3D-shape point cloud will be used to decode its ID.
}%
 \label{fig:detector}%
\end{figure*}

\section{Tag Detection}
\label{sec:Detection}
This section provides the individual steps for detecting potential markers and
examining their validity. The overall pipeline is shown in Fig.~\ref{fig:pipline}. To
localize potential \lidarts within the point cloud, the first step is to find
features. The features are then grouped into distinct
\emph{clusters}\footnote{Clustering features instead of clustering directly on a
\lidar scan is critical to achieve real-time applications.}. Most of these clusters
will not contain tags. Therefore, it is essential to validate whether a cluster
contains a \lidart or not.
%, see Sec.~\ref{sec:validation}.

% How the LiDAR returns are associated with each cluster is then
% explained to down select to a much smaller set of clusters that may
% contain valid \lidartsN.


% \begin{algorithm}[b]
% \caption{}
% \hspace*{\algorithmicindent} \textbf{Input:} Queues of point clouds, size of fiducial markers\\
% \hspace*{\algorithmicindent} \textbf{Output:} IDs and poses of LiDARTags
% \jkh{Added output, please check again}
% \begin{algorithmic}[1]
% \Procedure{LiDARTag Detection}{} 
%     \State LiDAR characteristics analysis [\ref{sec:analysis}] \\ \Comment{Only do it once}
%     \While{Point cloud queue != 0}
%         \State Edge detection [\ref{sec:edge}] 
%         \State Clustering [\ref{sec:clustering}] 
%         \State Validation [\ref{sec:validation}] 
%         \ForAll {Valid clusters}
%             \State Marker Extraction [\ref{sec:validation}] 
%             \State Pose Estimation [\ref{sec:pose_estimation1}] and  [\ref{sec:pose_estimation2}]
%             \State Weighted Gaussian Voting [\ref{sec:weighted_voting}]
%             \State Decoding [\ref{sec:decoding}]
%         \EndFor
%     \EndWhile
% \EndProcedure
% \end{algorithmic}
% \label{alg:lidartag}
% \end{algorithm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{\del{Tag Detection}}
% \label{sec:detection}
% \del{\lidart detection is the core of the LiDARTag system. To localize potential \lidarts
% within the point cloud, the first step is to apply edge detection. The edge points
% are then grouped into distinct \emph{clusters}. Most of these clusters will not
% contain tags. How the LiDAR returns are associated with each cluster is then
% explained in order to down select to a much smaller set of clusters that may contain
% valid \lidartsN. In Fig. \ref{fig:tag_explain}, to extract the fiducial marker
% rigidly attached to on a freestanding object, another edge detection is deployed. The
% last step, the partial pose (except the rotation about the z-axis) of the payload is
% estimated. The full rotation estimation will be addressed in
% Sec.~\ref{sec:pose_estimation2} and Sec.~\ref{sec:decoding}.}


\subsection{Feature Detection}
\label{sec:edge}
As mentioned in Sec.~\ref{sec:lidarVScamera}, images are very structured in that the
vertical and horizontal pixel-pixel correspondences are known. Consequently, various
kinds of 2D kernels~\cite{canny1987computational} can be applied for edge detection.
However, unlike images, raw \lidar point clouds are unstructured in that even if we
have the indices of all points in each beam, we do not know the vertical point-point
correspondences. 

Therefore, to find a feature in a point cloud, an edge point is
defined as discontinuities in distance. Inspired by the point
selection method in LeGO-LOAM~\cite{legoloam2018}, a point is defined as a
feature if it is an edge point, and its consecutive $n$ points are not edge
points (similar to plane features in LeGO-LOAM). Given consecutive $n+1$ points, we
choose to use a 1D kernel to compute spatial gradients at each point to find edge
points. Let $p_{i,m}$ be the $i^{\text{th}}$ point in the $m^{\text{th}}$ beam so that the gradient of distance $\nabla D(p_{i,m})$ can be defined as
\begin{equation}
\label{eq:GD}
         \nabla D(p_{i,m}) = \|p_{i+l,m} - p_{i,m}\|_2 - \|p_{i-l,m} - p_{i,m}\|_2, 
\end{equation}
where $\ell$ is a design choice (here, $\ell=1$). If $\nabla D(p_{i,m})$ at a point
exceeds a threshold $\zeta$, we then consider $p_{i,m}$ as a possible edge point.
Using distance gradients requires a \lidart being $\zeta$
away from the background. For speed in real time application, we do not apply
further noise smoothing, edge enhancement, nor edge localization. Finally, if
there is only one edge point in the consecutive $n+1$ points ($n=2$ in this
paper), then the edge point is considered as a feature.



\subsection{Feature Clustering}
\label{sec:clustering}
After determining the features in the current point cloud, we group them
into clusters using the single-linkage agglomerative hierarchical clustering
algorithm\footnote{We chose this clustering algorithm because the number of
        \lidarts is unknown. Therefore, algorithms like K-Means Clustering cannot be
used.}~\cite{johnson1967hierarchical, lloyd1982least}. As indicated in
Sec.~\ref{sec:lidarVScamera}, \lidar returns are not uniformly distributed in angles
or distance. The linkage criteria, therefore, considers the $x$-$y$ axes and the
$z$-axis differently: signed Manhattan distance is chosen for the $x$-$y$ axes, and
ring numbers are selected for the $z$-axis. Similarly, boundaries of a cluster are
defined by the four center points of a cuboid's faces and maximum/minimum ring
numbers, as shown in Fig.~\ref{fig:cluster}. The algorithm loops over each
feature, either linking it to an existing cluster and updating its boundaries,
or creating a new cluster. 

\begin{remark}
    \lidar rings are determined by the elevation angle of an emitter.
    Most existing \lidars provide not only $(x,y,z,i)$ values, but also a ring
    number of a data point. If ring numbers are not available and there exists only one
    rotation axis in the \lidarN, a ring number can be simply regressed against
    elevation angle by taking the \lidarN's ring numbers as a discrete set of
    corresponding elevation angles, in which the number of elevation angles is the
    same as the number of beams of the \lidarN. The elevation angle of a data point
    can be computed as 
    $$\arctan\left({\frac{z}{\sqrt{x^2+y^2}}}\right).$$
    We use
    this method to regress ring numbers for the Google Cartographer dataset. For more
    detail, see our implementation on GitHub~\cite{githubLiDARTag}.
\end{remark}



The boundaries $(b_1,\cdots,b_4, r_{max}, r_{min})$ of a cluster are the
maximum/minimum $x$, maximum/minimum $y$ and maximum/minimum ring numbers among all
features in the cluster. When a new cluster is created from a feature
$p^k=(x, y, z, i, r)$, the four center points of the faces are defined as $(x\pm
\tau, y\pm \tau)$, with $\tau = t\sqrt{2}/4$ for the
$(b_1,\cdots,b_4)$. The $r_{max}$ and $r_{min}$ are defined in terms of the ring numbers $r$, as shown in
Fig.~\ref{fig:cluster}. The linkage criteria $L(p^k,c_j)$ between a feature
$p^k$ and a cluster $c_j$ is 
\begin{equation}
\begin{cases}
 \label{eq:linkage}
&\min (b_i^k - \tau)  \leq p^k \leq \max (b^k_i + \tau), ~\forall i=1, \cdots,4\\
&r_{min}-1  \leq r \leq r_{max}+1,
\end{cases}
\end{equation}
where the first line is the signed Manhattan distance for the $x$-$y$ axes and the second is the ring number for the $z$-axis. If both
conditions are met, the feature is linked to the cluster. The corresponding boundaries
are updated, if necessary. Due to this linkage criteria, a \lidart
requires $\tau = t\sqrt{2}/4$ clearance around it to
avoid false linkage, and based on preliminary testing, we also impose that the topmost beam on the \lidart should be above $3/4$ of
the target, as indicated by the red region in Fig.~\ref{fig:TopMostBeam}. 

\begin{remark}
    We chose not to use a k-d tree structure~\cite{bentley1975multidimensional}
    because the number of features and the resulting clusters are not large enough to
    benefit from the data structure. The construction time of the tree could overtake 
    the querying time.
\end{remark}

\begin{figure}[t]%
\centering
\label{fig:cluster}%
\includegraphics[width=0.7\columnwidth]{ClusterBoundaries.png}%
\caption[]{This figure shows the initial state of a cluster, in which has only single
    one feature. A cluster is defined as a cuboid in $\realnumbers^3$. When a feature
    fails at linkage, a cluster will be created and centered at itself
$(x,y,z)$ with four boundaries $(x\pm\tau, y\pm\tau, z)$ for the $x$-$y$ axes, where $\tau$ is
$t\sqrt{2}/4$, as well as the maximum ring number and the minimum ring number for the
$z$-axis.
}%
\label{fig:cluster}%
\end{figure}

\begin{figure}[t]%
\centering
\subfloat[]{%
\label{fig:PoseIllustration}%
\includegraphics[width=0.45\columnwidth]{PoseIllustration.png}}%
\hspace{15pt}%
\subfloat[]{%
    \label{fig:TopMostBeam}%
\includegraphics[width=0.45\columnwidth]{TopMostBeam.png}}%
\caption[]{\subref{fig:PoseIllustration} describes the coordinate system of the
    fiducial marker. \subref{fig:TopMostBeam} indicates that the first beam hitting the
\lidart should be at least $3/4$ above target, outlined as the red region.
}%
\end{figure}


% If \eqref{eq:linkage} is true for $i^{\text{th}}$ cluster $c^i$,
% then add the edge to the cluster and update the corresponding cluster boundaries if necessary.
%\rha{I don't really follow this. You compute the minimum distance along any axis between the new point and all clusters' boundary points? Then if any are less than 0, you add it to that cluster? What happens if more than one distance is less than 0? What does a distance less than 0 mean?} 
%\bh{It's a "signed distance". I saw people use signed euclidean distance so I just use signed Manhattan distance. We want a point belongs to a cluster not only because the point is close to the cluster but also inside the cluster. The situation shouldn't not happened. What clusters actually do is split the environment into blobs and blobs contains detected edges from left to right.}

% \begin{algorithm}[t]
%     \hspace*{\algorithmicindent} \textbf{Input:} Edges and size of fiducial markers \\
% \hspace*{\algorithmicindent} \textbf{Output:} Collection of clusters of a scan of
% point clouds 
% \caption{}
% \begin{algorithmic}[1]
% \Procedure{Clustering}{} 
%     \ForAll {edges}
%         \If{Cluster queue==0}
%                 \State Create a new cluster with the edge
%                 \State Update boundaries with the edge
%         \Else
%             \ForAll {cluster}
%                 \If{!linkage}
%                     \State Create a new cluster with the edge
%                     \State Update boundaries with the edge
%                 \Else 
%                     \State Update boundaries with the edge
%                 \EndIf
%             \EndFor
%         \EndIf
%     \EndFor
%     % \If{$condition = True$}
%     %     \State Do this
%     %     \If{$Condition \geq 1$}
%     %     \State Do that
%     %     \ElsIf{$Condition \neq 5$}
%     %     \State Do another
%     %     \State Do that as well
%     %     \Else
%     %     \State Do otherwise
%     %     \EndIf
%     % \EndIf
% \EndProcedure
% 
% \end{algorithmic}
% \label{alg:hierarchical}
% \end{algorithm}

\subsection{Cluster Validation}
\label{sec:validation}
At this point, we have grouped the features into clusters as shown in
Fig~\ref{fig:edges}. In practice, few (possibly none) of the clusters will contain a
valid tag and thus it is important to be able to eliminate clusters that are clearly
invalid. To do so, we first used the point cloud data to fill in LiDAR returns between the features of a cluster, as
shown in Fig. \ref{fig:filled}. 
% \add{This section describes validation steps before pose estimation and decoding,
% more validation steps are described in ~\bh{sec:PoseValidation}}

Inspired by AprilTag~\cite{olson2011apriltag,wang2016apriltag},
tag-family-based heuristics are used to validate a cluster: number of points
$\eta$ and number of features $\psi$ in the cluster. Another geometry-based heuristic is also
deployed: the outlier percentage $(\kappa)$ of a plane fitting process. To save
computation time, if any of the above processes fails, the cluster is marked as
invalid and does not proceed to the next stage of validation. The first two values are
determined by what type of tag family is chosen. Shown in Fig.~\ref{fig:MarkerExample}
is a tag family which contains 16 bits. 


A lower bound on the number of points in a cluster is determined by how many bits
are contained in the fiducial marker. If the payload is $d \times d$, the LiDARTag
including boundaries is $(d+4) \times (d+4)$. If we assume a minimum of five returns
for each bit in the tag, then the minimum number points in a valid cluster is
\begin{equation}
    \eta \ge 5(d+4)^2.
\end{equation}

On the other hand, an upper bound is determined by the distance from the \lidar
to the marker and its size $t$. Given a tag at distance $D$, the maximum number of
returns on the marker happens when it directly faces to the \lidar and can be
computed as:
\begin{equation}
    M \frac{t\sqrt{2}}{D\sin{\theta}},
\end{equation}
where $\theta$ is the horizontal resolution of the \lidarN, $M$ is the number of
rings hitting on the tag, and $t\sqrt{2}$ is the diagonal length of the tag, as shown
in Fig.~\ref{fig:TopMostBeam}.


The boundaries of the payload can be detected by an intensity gradient, 
\begin{equation}
        \nabla I(p_{i,m}) = 
        |p_{i+\ell,m}^I - p_{i,m}^I| - |p_{i-\ell,m}^I - p_{i,m}^I|,
        \label{eq:GI}
\end{equation}
where $\ell$ is also a design choice (here, taken as one), and $p_{i,m}^I$ is the
intensity value of the $i^{\text{th}}$ point on the $m^{\text{th}}$ ring. An
example of detected boundary points is shown in Fig.~\ref{fig:boundary}.
If $\nabla
I(p_{i,m})$ exceeds a threshold, then $p_{i,m}$ is a payload edge point. To
successfully decode a tag, we will need at least one ring on each row of the payload.
Hence, the minimum number of payload edge points is
\begin{equation}
    \psi \ge 2(d+2).
    \label{eq:psi}
\end{equation}
Finally, we apply a plane fitting process to the remaining clusters. If the percentage
of outliers of the plane fitting is more than $\kappa$ (chosen as $0.05$), the
cluster is considered invalid.

The above heuristics allow us to extract a potential fiducial marker from the \lidart
through features in both cluttered indoor and spacious outdoor
environments. The next step is to estimate the pose of the marker.





\begin{figure}[t]%
\centering
\includegraphics[width=0.8\columnwidth]{IdealFrame.png}%
\caption[]{
This conceptual figure illustrates the proposed method to estimate a \lidartN's
pose. The target’s coordinate frame is defined as the mean of the four vertices 
$(\tilde{X}_1, \cdots, \tilde{X}_4)$ and the template of known geometry is defined 
by $(\bar{X}_1, \cdots, \bar{X}_4)$ with depth $\epsilon$ at the \lidar origin.
The rigid-body transformation $H_T^L$ (black arrow) pulls back the target’s
point cloud to the template. The actual pose of the \lidart is estimated by
\eqref{eq:Pose} using the inverse transformation $H_T^L$ (green arrow).
}%
\label{fig:IdealFrame}
\end{figure}




==> Detector_.tex <==
\section{Tag System}
\label{sec:Methodology}
This section describes the essential components of designing and using a LiDAR-based tag system. In particular, it addresses how the unstructured point cloud from a LiDAR results in different considerations in the selection of a LiDARTag than standard fiducial tags used with cameras. The section also outlines how to detect a LiDARTag and how to 
decode the tag. The overall pipeline used in detecting and decoding the tag is shown in  Fig.~\ref{fig:pipline}.

\begin{figure*}[t]
    \includegraphics[width=\linewidth]{pipeline.png}
    \caption{This system contains three parts: detection, classifying/weighting and
    decoding. The detection take a whole scan of point clouds up to 1.2m points from
    a Velodyne Ultra Puck and output collections of payload points along with partial
poses of LiDARTags. Next step classify payload points into different bits and
use the proposed Gaussian weighted to assign weight of voting based on the location of
a point. In the second step, the pose of tag is completed up 90 degree. The final task is to 
read the bits from the payload field and loop up from a hash table. By rotating payload
field, we can complete full rotation.}
    \label{fig:pipline}
\end{figure*}

\subsection{LiDAR Point Clouds vs Camera Images}

Images are very structured...uniform pixel grids and fixed number of points in an image

LiDAR has accurate distance, hence using distance for edge detection of the tag becomes interesting.

LiDAR returns consist of x-y-z coordinates and intensity.

Density of measured values on a tag will be much lower with LiDAR than with today's cameras

Number of points collected varies in each scan and for each beam. Hence LiDAR returns cannot be assumed uniformly distributed in angle or distance. A high contrast difference in the target can result in missing returns and hence large gaps between returns. Consequently, the same index number of returns from two different beams does not correspond to a fix geometric relationship. 

For a 15 cm x 15 cm "payload" at a distance of 2 m -----give idea of the number of returns one can expect vs a typical camera's number of pixels. 11,642

Number of points affected by temperature.

Because pixels are in a uniform grid, 

%Unaffected by lighting<-----red herring 

LiDARs are different from cameras. Once selected a resolution, 
cameras have fixed number of pixels for all the images. 
% A scan of point cloud from LiDAR is usually expressed in beam. 
Given a same beam number, 
we still have much different amount of points in different LiDAR
such as Velodyne HDL-32E and Velodyne ULTRA PUCK \red{CITE?}. Point clouds from 
the same LiDAR do not have the same amount of points in each scan. 
Moreover, it also depends on the weather: if 
the weather is warm/hot, the size of the point clouds are smaller; larger if cold. 
Thus, it is critical to analyze the LiDAR device Sec. \ref{sec:analysis} first every time it starts.

\begin{algorithm}[b]
\caption{}
\hspace*{\algorithmicindent} \textbf{Input:} Queues of point clouds, size of fiducial markers\\
\hspace*{\algorithmicindent} \textbf{Output:} IDs and poses of LiDARTags
\jkh{Added output, please check again}
\begin{algorithmic}[1]
\Procedure{LiDARTag Detection}{} 
    \State LiDAR characteristics analysis [\ref{sec:analysis}] \\ \Comment{Only do it once}
    \While{Point cloud queue != 0}
        \State Edge detection [\ref{sec:edge}] 
        \State Clustering [\ref{sec:clustering}] 
        \State Validation [\ref{sec:validation}] 
        \ForAll {Valid clusters}
            \State Marker Extraction [\ref{sec:validation}] 
            \State Pose Estimation [\ref{sec:pose_estimation1}] and  [\ref{sec:pose_estimation2}]
            \State Weighted Gaussian Voting [\ref{sec:weighted_voting}]
            \State Decoding [\ref{sec:decoding}]
        \EndFor
    \EndWhile
\EndProcedure
\end{algorithmic}
\label{alg:lidartag}
\end{algorithm}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Tag Design or Selection}
\label{sec:selection}

So that distance can be used to determine edges when seeking to isolate a LiDARTag in a 3D point cloud, a LiDARTag is assumed to consist of a planar fiducial marker rigidly  attached to a freestanding 3D object, such as a stop sign. In particular, in this paper, the fiducial marker cannot be attached to a wall.  

The planar fiducial marker
carry real information and is attached on the sign, as
shown in Fig. \ref{fig:LiDARTag}.
It can be chosen from any types of fiducial markers that
with clear black and white boundaries such as apriltag 1-3~\cite{olson2011apriltag}~\cite{wang2016apriltag}
\cite{krogiusflexible}, ARTag~\cite{fiala2005artag}~\cite{fiala2005comparing}, or 
InterSense~\cite{naimark2002circular} but not CyberCode~\cite{rekimoto2000cybercode}, Cho et.al~\cite{cho1998multi} 
nor CALTag~\cite{atcheson2010caltag}. The summary of the discussed tag families are 
shown in Fig. \ref{fig:tag_family}. 

\begin{figure}[t]%
\centering
\subfigure[][AprilTag 2]{%
\includegraphics[width=0.3\columnwidth]{apriltag.jpg}}%
\hspace{8pt}%
\subfigure[][ARTag]{%
\includegraphics[width=0.29\columnwidth]{artag.png}}%
\hspace{8pt}%
\subfigure[][InterSense]{%
\includegraphics[width=0.3\columnwidth]{InterSense.png}}\\
\hspace{8pt}%
\subfigure[][Cybercode]{%
\includegraphics[width=0.3\columnwidth]{cybercode.png}}%
\hspace{8pt}%
\subfigure[][Cho et.al]{%
\includegraphics[width=0.3\columnwidth]{colortag.png}}%
\hspace{8pt}%
\subfigure[][CALTag]{%
\includegraphics[width=0.3\columnwidth]{caltag.png}}%
\caption[]{The first row can be used as fiducial markers in LiDARTags because they
have clear black and white boundaries. However, the second row is not applicable due
to not containing clear black and white boundaries.}%
\label{fig:tag_family}%
\end{figure}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{LiDAR Characteristics Analysis}
\label{sec:analysis}
As mentioned in Sec. \ref{sec:intro}, a scan of point clouds from a Velodyne 32-beam Ultra Pack 
is up to 1.3 million points. However, actual points on a payload are spare. 
A scan of point clouds from a LiDAR device is usually made of many beams. For example, a scan of 
point clouds from Velodyne 32-beam is made of the 32 beams of points.
From our experience, the characteristics of LiDAR devices is challenging for an algorithm to work well:
\begin{enumerate}
    \item The number of points on each beam is different.
    \item The number of point in each scan is different.
    \item The number of points is also greatly influenced by environmental factors 
          such as weather, temperature.
    \item Irregular/inconsistent points tend to appearing more if great change of intensity happens, as
        shown in Fig. \ref{fig:irregular}.
\end{enumerate}

Inconsistency and irregularity mentioned above vastly challenge the robustness of a system.
In this analysis, our purpose is to let the detector, described in Sec. \ref{sec:detection}, to 
observe the characteristics of this specific LiDAR at this moment, at this weather, 
how many points are in a scan, how many points on each beam so as to help the 
detector accurately determine if a cluster is valid or not as described in 
Sec. \ref{sec:validation}. Thus, we create two tables: a point table that records how
many points on each beam and another table to record each scan of the average, maximum, minimum size
of point clouds. Note, this only need to be done one time at the every beginning of detection.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Tag Detection}
\label{sec:detection}
Tag detection is the core of the LiDARTag system. It consists of several steps. The first 
step is the edge detection in \ref{sec:edge}: finding where all potential LiDARTags are. 
The second step is to classify edges into different clusters in \ref{sec:clustering} and 
then validate each cluster \ref{sec:validation}. Up to this points, we are all dealing 
with edges. Next step, we fill in points into each cluster
in order to validate each cluster and also to find a fiducial marker, which includes boundaries marked
in red and an actual payload marked in green as shown in Fig. \ref{fig:tag_explain}. 
After validation, the remaining clusters are candidates of 
being actual LiDARTags. To extract a payload, another edge detection is applied. 
The last step, the partial pose (translation, pitch, yaw) of the payload will be estimated. 
The full roll angle estimation will be addressed in Sec. \ref{sec:pose_estimation2} and Sec. 
\ref{sec:decoding}.

\begin{figure}[t]%
\centering
\subfigure[][LiDARTag]{%
\label{fig:3dtag}%
\includegraphics[width=0.25\columnwidth]{3dlidartag.png}}%
\hspace{25pt}%
\subfigure[][AprilTag 2 as fiducial markers for a LiDARTag.]{%
\label{fig:tag_explain}%
\includegraphics[width=0.47\columnwidth]{tag_explain.png}}%
\caption[]{\subref{fig:3dtag} shows a possible LiDARTag, consisting of two parts: a 3D sign and
    a fiducial marker. \subref{fig:tag_explain} A fiducial marker can be anything with 
    clear black and white boundaries as shown in Fig. \ref{fig:tag_family}. We use
AprilTag as our fiducial markers in this paper.}%
\label{fig:LiDARTag}%
\end{figure}



\subsubsection{Edge Detection}
\label{sec:edge}
In images, all pixels are aligned: the number of pixel in every column are all the same;
the same applied to rows. In other words, the vertical pixel-pixel corresponds are known; 
therefore various kinds of 2D kernels~\cite{canny1987computational} can be applied for 
edge detection. 

However, unlike images, point clouds we have are unstructured and a number of points 
on each beam are not the same, which means points are not aligned even we have index of 
all points in a beam. Since we do not have vertical point-point correspondence in point clouds, we 
choose to use 1D kernel to compute spatial and intensity gradients at every point to find edges, 
which are defined as discontinuities in both intensity and depth.
Given the $i^{\text{th}}$ point $p_i$ at position $p_i^D$ and intensity $p_i^I$,
the gradient of intensity ($|\nabla I(p_i)|$) and gradient of depth ($|\nabla D(p_i)|$)
is defined follow:

\begin{align}
        |\nabla I(p_i)| &= max(||p_{i+2}^I - p_{i}^I||_2,\ 
                         ||p_{i-2}^I - p_{i}^I||_2) \label{eq:GI}\\
        |\nabla D(p_i)| &= max(||p_{i+2}^D - p_{i}^D||_2, \ 
                        ||p_{i-2}^D - p_{i}^D||_2) \label{eq:GD}
\end{align}
where $I$ is the intensity value and $D$ is the depth difference. If both
$\nabla I(x,y,z,I)$ and $\nabla D(x,y,z,I)$ at a point exceed thresholds,
we then consider a possible edge point. Due to numerous number of points and aiming
for real time application, we do not apply further noise smoothing, edge enhancement
nor edge localization.


\subsubsection{Cluster Grouping}
\label{sec:clustering}
After getting all edges in the current point cloud, we need to group the \emph{edges}
into different clusters. However, due to not knowing how many clusters nor how many
tags we have in the scene and for memory efficient, a slightly modified version of 
single-linkage agglomerative hierarchical clustering~\cite{johnson1967hierarchical} with 
signed Manhattan distance metrics is applied, as shown in Algorithm \ref{alg:hierarchical} 
and Fig. \ref{fig:cluster}. 

\begin{figure}[t]%
\centering
\subfigure[][Cluster boundaries]{%
\label{fig:cluster}%
\includegraphics[width=0.5\columnwidth]{cluster.png}}%
\hspace{8pt}%
\subfigure[][LiDARTag pose definition]{%
\label{fig:partialPose}%
\includegraphics[width=0.45\columnwidth]{partialPose.png}}%
\caption[]{\subref{fig:cluster} shows a single point cluster. A cluster is defined as
    a cuboid in $\realnumbers^3$. When a point fails at linkage, a cluster will be
    created and it is centered at itself $(x,y,z)$ with boundaries 
$(x\pm\tau, y\pm\tau, z\pm\tau)$, where $\tau$ is (tag size)/4. \subref{fig:partialPose}
show a definition of a LiDARTag, which is fully defined by a fiducial marker on it.}%
\label{fig:}%
\end{figure}

A cluster is defined as a cube in $\realnumbers^3$ space. Boundaries of a cluster are
defined by 6 points, as shown in \ref{fig:cluster}. The algorithm 
contains two steps: checking all existence clusters and either create a new one or 
update a existing cluster. If a point is \emph{linked} to a cluster that has been created, 
then add the point into the cluster and also update the boundaries of the cluster if
necessary. If a point fails linking to any existing clusters, then create a new cluster
centered at its own coordinate $(x,y,z)$ with boundaries of 
$(x\pm \tau, y\pm \tau, z\pm \tau)$ and $\tau = \text{(tag size)}/4$.
In Fig. \ref{fig:cluster}, the red point is the point that fails linking to any clusters
and the boundaries are ${b_i|i=1,...,6}$. 
To decide if a point is within a cluster or not, called the linkage criteria, a distance metric 
is required. In this work, the signed Manhattan distance metric is used and linkage
criteria $L(p,c_i)$ between a point $p$ and a cluster $c^i$ is defined as follow:


\begin{equation}
    % D(\p,\c) = \min_{k=1,...,6}(\p-\b[][k]) = \min_{i=x,y,z} (\p[i] - \b[i][k]), 
    L(p,c_i) \coloneqq \min_{\substack{k=x,y,z\\ m=1,...,6}} (p_k - b_k^m), 
\end{equation}
where $b_k$ are boundaries points of a cluster.
Assuming N clusters, if $\min_{i,...,N} L(p, c_i)<0$, 
then add to and update the corresponding cluster; otherwise, create a new cluster.

\begin{algorithm}[t]
    \hspace*{\algorithmicindent} \textbf{Input:} Edges and size of fiducial markers \\
\hspace*{\algorithmicindent} \textbf{Output:} Collection of clusters of a scan of
point clouds 
\caption{}
\begin{algorithmic}[1]
\Procedure{Clustering}{} 
    \ForAll {edges}
        \If{Cluster queue==0}
                \State Create a new cluster with the edge
                \State Update boundaries with the edge
        \Else
            \ForAll {cluster}
                \If{!linkage}
                    \State Create a new cluster with the edge
                    \State Update boundaries with the edge
                \Else 
                    \State Update boundaries with the edge
                \EndIf
            \EndFor
        \EndIf
    \EndFor
    % \If{$condition = True$}
    %     \State Do this
    %     \If{$Condition \geq 1$}
    %     \State Do that
    %     \ElsIf{$Condition \neq 5$}
    %     \State Do another
    %     \State Do that as well
    %     \Else
    %     \State Do otherwise
    %     \EndIf
    % \EndIf
\EndProcedure

\end{algorithmic}
\label{alg:hierarchical}
\end{algorithm}

\subsubsection{Cluster Validation and Fiducial Marker Extraction}
\label{sec:validation}
We have grouped \emph{edges} into different clusters. To validate clusters, we fill
in points between edges as shown in Fig. \ref{fig:filled}, 
i.e. a complete LiDARTag has been recovered from edges. 
Two types of validation are considered: number of points in a cluster,
called $\eta$, and edges \emph{inside} of the cluster (not including boundary of the cluster),
called $\psi$. 

\begin{figure}[t]%
\centering
\subfigure[][A full scan of point clouds.]{%
\label{fig:full_scan}%
\includegraphics[width=0.45\columnwidth]{fullScan.png}}%
\hspace{8pt}%
\subfigure[][Edges of a full scan point clouds.]{%
\label{fig:edges_full_scan}%
\includegraphics[width=0.47\columnwidth]{edges.png}}\\
\hspace{8pt}%
\subfigure[][Cluter of LiDARTag.]{%
\label{fig:edges}%
\includegraphics[width=0.4\columnwidth]{tag_edges.png}}%
\hspace{14pt}%
\subfigure[][Filled LiDARTag.]{%
\label{fig:filled}%
\includegraphics[width=0.46\columnwidth]{filledCluster.png}}\\
\subfigure[][Boundaries of a fiducial marker marked in red.]{%
\label{fig:fiducial_edges}%
\includegraphics[width=0.44\columnwidth]{fiducialEdge.png}}%
\hspace{8pt}%
\subfigure[][Weighted Gaussian voting visualization.]{%
\label{fig:color_points}%
\includegraphics[width=0.47\columnwidth]{color_points.png}}%
\hspace{8pt}%
\caption[]{Intermediate steps of the LiDARTag system. The system takes a full scan
    point cloud in \subref{fig:full_scan} and apply edge detection as defined in 
    \eqref{eq:GI}) and \eqref{eq:GD} as in \subref{fig:edges_full_scan}. Group \emph{edges} into
different clusters and \subref{fig:edges} shows a cluster of a LiDARTag. To validate
if a cluster, original points from a full scan of point clouds are filled back in
\subref{fig:filled}. After validation, another edge detection is applied to find
boundaries of a \emph{fiducial marker} in \subref{fig:fiducial_edges}. In \subref{fig:color_points} 
shows classified points of a \emph{fiducial marker}. Points of a \emph{fiducial
marker} have been classified into different grids by projecting them back to a
known coordinate and reweight each point from a Gaussian distribution (red circles) 
by it location \emph{inside} a grid.}%
\label{fig:detector}%
\end{figure}

Both types of constrain are determined by what type of tag family is chosen. Shown in Fig.
\ref{fig:tag_explain} is a tag family $d^2$, contains $d^2$ bits. For the first type of
constrain, the size of a fiducial marker is $(d+2)^2$. The whole area of a LiDARTag is roughly 
$(d+4)^2$. To achieve accurate decoding result, we require minimum returns on each bit being 6. 
Therefore, the number of points of a valid, reliable cluster should at least have
\begin{equation}
    \eta \ge 6(d+4)^2.
\end{equation}

To evaluate the second type of constrain, another edge detection is applied. However,
unlike edge detection mentioned in Sec. \ref{sec:clustering}, we only apply
\eqref{eq:GI} to find edges of a fiducial marker as shown in Fig. \ref{fig:fiducial_edges}.
We require at least one beam on each row to be able to successfully 
decode the payload, i.e. edges of the fiducial marker should at least:
\begin{equation}
    \psi \ge 2d.
\end{equation}

While evaluating the second constrains, we have extracted the fiducial marker
from the 3d tag by applying another edge detector. The next step is to estimate the
pose of the fiducial marker.

\subsubsection{Partial Pose Estimation}
\label{sec:pose_estimation1}
The coordinate of a LiDARTag is defined in Fig. \ref{fig:frame}.
The most convenient way of representing a pose of a LiDARTag is using a point
$\mu$ $(x,y,z)$ and a quaternion q $(q_w, q_x, q_y, q_z)$ where 
$\mu$ is the center of the \emph{fiducial marker} and 
q is rotation of the \emph{fiducial marker} as shown in Fig. \ref{fig:partialPose}.
In other words, a pose of a LiDARTag is fully defined by the \emph{fiducial marker}
attached to a LiDARTag. Given a set of $N$ points of a fiducial marker: 
\begin{equation}
    p_i|i=1, ..., N, \ p_i\in\realnumbers^3,
\end{equation}
The center of a LiDAR, $\mu$, is estimated as the mean of all the points $p$:
\begin{equation}
    \mu = \sum_{i=1}^{N}\frac{p_i}{N}.
    \label{eq:PCA_mu}
\end{equation}

The rotation of a LiDARTag, q, is estimated by the normal vector of the given points.
The normal vector is estimated from principal components analysis
(PCA)~\cite{price2006principal}. The first two components of PCA are the two vectors
aligning on a fiducial plane. The least components is the normal vector that we are
looking for.

The PCA can be applied as followed:
% The centroid of the given point has been 
\begin{enumerate}[(i)]
    \item Compute centroid point $\mu$, which has been calculated 
        in \eqref{eq:PCA_mu}.
    \item Compute zero mean points $y_i = p_i-\mu$.
    \item Apply SVD to $\Y = \textbf{U}\boldsymbol{\Sigma}\V[][\transpose]$.
\end{enumerate}
Then the normal vector of a fiducial marker is the last column of vector of
$\textbf{U}$. However, the normal vector cannot determine the roll angle of the
fiducial marker, which is addressed in Sec. \ref{sec:pose_estimation2}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Classification of points}
\label{sec:grouping}
We now have boundaries and points on a fiducial tag that has been done in Sec.
\ref{sec:validation}. To be able to decode a LiDARTag, color of a bit being white or
black is needed. Since a LiDARTag could be at any position and any orientation, we
need to project them back to a known plane so each point can be assigned to a
corresponding bit on the \emph{payload} of a fiducial marker, described in Sec.
\ref{sec:pose_estimation2}.

Due to sparsity of points on a LiDARTag, missing points and noisy
measurement we have, naively classifying based on location of a point is not enough.  
Weighted Gaussian voting is used to weight each point according to its location inside a grid, 
described in Sec. \ref{sec:weighted_voting}.


\subsubsection{Points Remapping}
\label{sec:pose_estimation2}
We want to estimate a homogeneous transformation $H$ with a translation $T$ and a rotation 
matrix $R$ from the LiDARTag coordinate to a hyper-coordinate as shown in Fig. \ref{fig:mapping}.
This problem can be formulated into a procrustes optimization problem~\cite{gower1975generalized}:
\begin{equation}
\Theta = \argmin_{\substack{\Omega \\ \text{s.t }\Omega^T\Omega=I}} ||\Omega A-B||_F.
\end{equation}

What we have are four corners and a center point of a fiducial marker as well as a known square 
with known vertex positions on a hyper-coordinate. Without loss of generality, $x_0$ is assumed at $(0,0,0)$. 
The translation $T$ can be formulate as:
\begin{align}
    x_0 &= Rp_0 + T , \ x_0=[0,0,0]^\transpose \nonumber\\
    T &= -Rp_0
\end{align}
The rest of the problem can be formulated as:
\begin{align}
    \left\|H\tilde{p_i}-x_i\right\|^2_2 &= \left\| \begin{bmatrix} R & T\\ \zeros & 1
        \end{bmatrix} \begin{bmatrix} p_i \\ 1 \end{bmatrix} - 
        \begin{bmatrix} x_i \\ 1\end{bmatrix}\right\|_2^2 \\
        &= \left\|Rp_i+T-x_i\right\|^2_2 = \left\|Rp_i^{\prime}-x_i\right\|^2_2,
\end{align}
\begin{align}
    \sum_{i=1}^4 \left\|H\tilde{p_i}-x_i\right\|^2_2 &= \sum_{i=1}^4
    \left\|Rp_i^{\prime}-x_i\right\|^2_2\\
                                                     &= \left\|
                                                     (Rp_1^{\prime}-x_1)\vdots\
                                                     \cdots \ 
                                                     \vdots(Rp_4^{\prime}-x_4)
                                                     \right\|_F^2 \\
                                                     &= \left\|R\P-\X \right\|^2_F.
\end{align}
where $\tilde{p_i} = [p_i \ 1]^\transpose$,  $p_i^{\prime} = p_i-p_0$, 
$\P=\begin{bmatrix} p_1^\prime& p_2^\prime&  p_3^\prime &p_4^\prime\end{bmatrix}$ 
and $\X=\begin{bmatrix} x_1& x_2&  x_3 &x_4\end{bmatrix}$.
The whole problem then becomes:
\begin{align}
    R^\ast = \argmin_{\substack{R \\ \text{s.t }R^TR=I}} \left\| R\P -\X\right\|_F^2.
\end{align}

By the procrustes optimization problem~\cite{gower1975generalized}\jkh{cited}
, we have a closed form solution:
\begin{align}
    M &= \X\P[][\transpose] = \U\Sigma\V[][\transpose] \\ 
    R^\ast &= \U\V[][\transpose].
\end{align}
The $R^\ast$ can be used to determine the roll angle of a normal vector that we had
calculated in Sec. \ref{sec:pose_estimation1}. However, the roll angle is only up to $90^{\circ}$,
i.e. whether a LiDARTag is at rotation of $0^\circ, 90^\circ, 180^\circ, 270^\circ$ still remains
unknown as shown in Fig. \ref{fig:codeword_rotation} and 
will be addressed in Sec. \ref{sec:decoding}.

\blue{can write more about how to classify.}


\begin{figure}[t]
  \centering 
  \includegraphics[width=0.9\columnwidth]{Mapping.jpg}
  \caption{Transform points on a fiducial marker to a known hyper-coordinate so the points 
  on the fiducial marker can be classifying into a corresponding bit.}
  \label{fig:mapping}
\end{figure}

\subsubsection{Weighted Gaussian Voting}
\label{sec:weighted_voting}
After remapping points back to the square on a hyper-coordinate, equally voting from
each point in each grid performs poorly results due to inconsistent/irregular points. 
The proposed weighted Gaussian voting technique captures the underlying distribution better.

We take a square with $(d+2)\times(d+2)$ grids with classified points marks
with different colors for an example. We form $d^2$
multivariate Gaussian distributions drawn in red circles as shown in Fig. \ref{fig:color_points}:
\begin{align}
    w_{p_i} &\sim \Ncal_k\left( \mu_k, \Sigma\right) \\
    \mu_k &= \begin{bmatrix} x_k\\ y_k\end{bmatrix}, \ \ \Sigma = \begin{bmatrix} \sigma^2 &0\\ 0 & \sigma^2\end{bmatrix}\\
    \sigma^2 &= \frac{\text{size of fiducial marker}}{4(d+2)},
\end{align}

    where $\mu_k$ is the center of $k^{\text{th}}$ grid drawn in white dots in Fig. \ref{fig:color_points},  $k=1,\ ...,\ (d+2)^2$ and
    covariance is a constant depending on the size of a fiducial marker. Given a point $p_i$ in 
    the $k^{\text{th}}$ grid, its weight $w_{p_i}$ is drawn from $\Ncal_k\left(
    \mu_k, \Sigma\right)$.

    Assume $N$ points in the $k^{\text{th}}$ grid. The possibility $P_k$ of the 
    $k^{\text{th}}$ grid being white or black is determined as follow:
    \begin{align}
        P_k = \frac{\sum_{i=1}^{N} w_{p_i}p_i^I}{\sum_{i=1}^{N} w_{p_i}},
    \end{align}
    where $p_i^I$ is the intensity value of the point $p_i$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Tag Decoding}
\label{sec:decoding}
After getting the codewords of $d^2$ bits on a payload, the way of decoding is the same manner of
AprilTag 1 and AprilTag 2~\cite{olson2011apriltag}~\cite{wang2016apriltag}. 
We have precomputed a hash table to stored the codebook of this tag family. While looking up a codewords
from a payload, the codewords will be rotated three times as shown in Fig. \ref{fig:codeword_rotation}
to find the rotation of $90^\circ, 180^\circ, 270^\circ$ of the code so we can fully
recover a roll angle.
As mentioned in the AprilTag 2 paper, a tag is identified as the code with
smallest hamming distance from the detected codewords on a payload. The decode system
can correct up to $\floor{(h-1)/2}$ and detect $h/2$ bit errors. For more detail on
decoding an AprilTag, we refer reader to Olson~\cite{olson2011apriltag}.

\begin{figure}[t]%
\centering
\subfigure[][Codeword is rotated $0^\circ$.]{%
\label{fig:codeword1}%
\includegraphics[width=0.4\columnwidth]{codeword1.jpg}}%
\hspace{12pt}%
\subfigure[][Codeword is rotated $90^\circ$.]{%
\label{fig:codeword2}%
\includegraphics[width=0.4\columnwidth]{codeword2.jpg}}\\
\subfigure[][Codeword is rotated $180^\circ$.]{%
\label{fig:codeword3}%
\includegraphics[width=0.4\columnwidth]{codeword3.jpg}}%
\hspace{12pt}%
\subfigure[][Codeword is rotated $270^\circ$.]{%
\label{fig:codeword4}%
\includegraphics[width=0.4\columnwidth]{codeword4.jpg}}%
\caption[]{Before decoding, estimated poses of roll angles are only up to $90^\circ$, which means
from \subref{fig:codeword1} to \subref{fig:codeword4}, estimated roll angles will be the
same. By rotating three times $(90^\circ, 180^\circ, 270^\circ)$, which results in 4 codewords
from \subref{fig:codeword1} to \subref{fig:codeword4}, 
while looking up for the correct id of a LiDARTag (only one of the four codewords is correct), 
we can recover the correct rotation of a roll angle.}%
\label{fig:codeword_rotation}%
\end{figure}


==> Experiments_pre.tex <==
% A) Cluttered vs spacious
% B) Pose accuracy -> plots and summary table
% C) Decoding accuracy -> plots and summary table
% D) Algorithm analysis
% -- a) general speed analysis, number of clusters -> similar to Tab 1 in the original paper
% -- b)  pose optimization: gradient, different solvers comparison
% -- c) decoding process:  parallel processing, matrix, vector, kd-tree analysis
% E) False positive rate from other datasets -> summary table
\section{Experimental Results}
\label{sec:results}
We now present experimental evaluations of the proposed LiDARTag. All experiments are
done with a 32-beam Velodyne Ultra Puck and an Intel RealSense camera as shown in
Fig. \ref{fig:torso} rigidly attached to the torso of a Cassie-series bipedal robot.
The \lidart system runs on a laptop equipped with Intel$^\text{\textregistered}$
Core$^{\text{TM}}$ i7-7700HQ CPU @ 2.80 GHz. 

The evaluation is separated into  

To evaluate pose accuracy, a motion capture system developed by Qualisys is used as a
proxy for ground truth poses. The setup consists of 30 motion capture cameras with
markers attached to tags, a LiDAR and a camera. Datasets are collected at various
distances and different angles. Each of the datasets contains images (20 Hz) and
scans of point clouds (10 Hz). We use the Robot Operating System
(ROS)~\cite{quigley2009ros} to communicate and synchronize between sensors. 


To 


\begin{figure}[t!]%
\centering
\subfloat{%
\label{fig:LiDAR_static}%
\includegraphics[width=0.5\columnwidth]{lidartag_static_error.jpg}}%
\subfloat{%
\label{fig:AprilTag_static}%
\includegraphics[width=0.5\columnwidth]{apriltag_static_error.jpg}}%
\caption[]{Plots of estimation error for a static tag, LiDAR and camera.
}%
\label{fig:LiDAR_results}%
\squeezeup
\end{figure}

\begin{figure}[t!]%
\centering
\subfloat{%
\label{fig:LiDAR_moving}%
\includegraphics[width=0.5\columnwidth]{lidartag_moving.jpg}}%
\subfloat{%
\label{fig:AprilTag_moving}%
\includegraphics[width=0.5\columnwidth]{apriltag_moving.jpg}}%
\caption[]{Estimated position and orientation when the LiDAR and camera are moving and the tag is stationary.}%
\label{fig:LiDAR_results_moving}%
\squeezeup
\end{figure}

%the accuracy while the LiDARTag remains still and move LiDAR back and froth. The
%orientation is a little noisy due to the bumpy ground, which caused instant jump while
%measuring. This could be improved by motion compensation.
% \begin{figure}[t]%
% \centering
% % \label{fig:sim_calibration}
% \includegraphics[trim=15 60 100 15, clip, width=0.90\columnwidth]{sim_results.jpg}
% \caption[]{Simulated results of calibration. The baseline is incremental mean (dashed-green) with batch size 30. The InEKF method with batch size 30 outperforms the baseline (dotted-purple). The sample
%     mean (solid-red) works the best; however, it cannot do incremental solutions.
%     Note, at the y-axis, it is log-scale of $\lVert\Log(X^{-1}_{\text{measurement}}X_{\text{truth}})\rVert_2$. 
% \mgj{I still think a Gauss-Newton (least squares) or even better an Iteratively Reweighted Least Squares (IRLS) solver sounds like a better estimator. The sample mean has access to all data and InEKF process them incrementally. So they're not really within the same class to compare them. Ross can run the Gauss-Newton solver for you.}}%
% \label{fig:calibration_results}%
% \end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Computational Time and Decoding Accuracy}
In this work, we choose a stop sign as our freestanding 3D object and AprilTag 2 as our fiducial markers, 
as shown in Fig. \ref{fig:LiDARTag}. 
To evaluate the computation time and decoding accuracy, we placed the torso at 2
meters away from a \lidart\ for both indoor and outdoor experiments.
The computation time of each step of the pipeline is shown in Table \ref{tab:accuracy}. 
Indoors, we have more edge points due to a cluttered environment. However, we have fewer
clusters indoor because detected edge points are closer to each other resulting in many of them being clustered together. The computation time in an outdoor environment 
was slower than indoor because we have more clusters to create and validate. 
In both environments, the system achieves real-time performance (at least 20 Hz).
The decoding accuracy in both environments is $99\%$. 

In the indoor and outdoor environments, the equal-weight decoding method fails to determine a codeword for $0.4152\%$ and $0.0822\%$ of the time; codeword are determined but the decoder cannot find a corresponding codeword from the codebook for $85.6055\%$ and $84.4984\%$ of the time; the decoder finds a wrong codeword for $13.9792\%$ and $15.4194\%$ of the time. All together, this amounts to $0.0001\%$ and $0.0000\%$ accuracy, indoor and outdoor, respectively.


The above work used tag16h5. Prior to settling on it, we
also tested other tag families 
in AprilTag 2, such as tag49h14 and tag25h10, with lower accuracy, due to the sparsity of our point clouds.  If the number of points in a grid, after the
remapping in Sec. \ref{sec:pose_estimation2}, is less than 5, it is considered a bad bit. 
Since the tag16h5 has a Hamming distance of 5, we allow up to 2 bad bits in a payload. 
If more than 2 bad bits are detected, the payload was rejected. 

In our work, we printed the AprilTags on A4 paper. Users could also print larger tags and use a larger Hamming distance to allow more bad bits, if the 2-bit limitation appears as a critical issue.

\begin{table*}[t!]
\caption{LiDARTag Accuracy and Computation Time. Unless it is mentioned, all times are reported in milliseconds. The number of points, number of edge points and number of clusters are the average of all scans. The decoding accuracy of the weighted Gaussian voting technique in both environments is $99\%$. Most of the computation time is spent on clustering edge points. Actual time spent on validation and other processes is relatively small. The accuracy of equal weight method is poor due to failed determination of a codeword, no existing codewords found in the codebook, or finding a wrong codeword.}
\vspace{-3pt}
\label{tab:accuracy}
\resizebox{1\textwidth}{!}{%
    \begin{tabular}{lllllll}
        \multicolumn{7}{c}{\textbf{Indoor}} \\ \midrule
        % \rowcolor[HTML]{C0C0C0} 
        \begin{tabular}[c]{@{}c@{}}Collecting \\ time\end{tabular} &
        \begin{tabular}[c]{@{}c@{}}No. Scans~~\end{tabular} &
        \begin{tabular}[c]{@{}c@{}}No. Points~~\end{tabular} &
        \begin{tabular}[c]{@{}c@{}}No. Edges~~\end{tabular} &
        \begin{tabular}[c]{@{}c@{}}No. Clusters~~~\end{tabular} &
        \begin{tabular}[c]{@{}c@{}}Accuracy of \\ Equal Weight\end{tabular}
        & \begin{tabular}[c]{@{}c@{}}Accuracy of \\ Gaussian
        Weight\end{tabular} \\ \midrule
        120 $\mathrm{sec}$ & 1240 & 53548 & 3813 & 779 & 0.0001\% & 99.6371\% \\ \midrule
        Clustering~~ & Validation~~ & Extraction~~ &
        Normal Vec.~~ & Decoding~~ &
        \multicolumn{2}{c}{Total computation time} \\ \midrule
        24.004 & 1.754 & 0.0271 & 0.0339 & 1.199
        & \multicolumn{2}{c}{29.496896 (33.9 Hz)} \\ \midrule 
        \multicolumn{7}{c}{\textbf{Outdoor}} \\ \midrule
        \begin{tabular}[c]{@{}c@{}}Collecting \\ time\end{tabular} &
        \begin{tabular}[c]{@{}c@{}}No. Scans\end{tabular} &
        \begin{tabular}[c]{@{}c@{}}No. Points\end{tabular} &
        \begin{tabular}[c]{@{}c@{}}No. Edges\end{tabular} &
        \begin{tabular}[c]{@{}c@{}}No. Clusters~~~\end{tabular} &
        \begin{tabular}[c]{@{}c@{}}Accuracy of \\ Equal Weight\end{tabular}
        & \begin{tabular}[c]{@{}c@{}}Accuracy of \\ Gaussian
        Weight\end{tabular} \\ \midrule
        266 $\mathrm{sec}$ & 3820 & 52477 & 2416 & 1757 & 0.0000\% & 99.7382\% \\ \midrule
        Clustering & Validation & Extraction &
        Normal Vec. & Decoding &
        \multicolumn{2}{c}{Total computation time} \\ \midrule
        38.096 & 4.741 & 0.0290 & 0.0319 & 1.202
        & \multicolumn{2}{c}{44.655821 (22.4 Hz)} \\ \bottomrule
    \end{tabular}
}
% \vspace{5pt}
% \caption*{}
\end{table*}
\vspace{-5pt}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{LiDARTag Pose Accuracy Evaluation}
\label{sec:pose_acc}
As described in Sec. \ref{sec:pose_estimation1}, \ref{sec:pose_estimation2} and shown
in Fig. \ref{fig:partialPose}, the LiDARTag pose ($\mu$ and $q$) is defined by the middle of a 
fiducial marker and the normal vector of a fiducial marker, respectively.
To evaluate pose accuracy of the proposed LiDARTag, we did two experiments. In the
first experiment, we held Cassie's torso in a fixed position, and recorded for 2 minutes. 
The results are shown in Fig. \ref{fig:LiDAR_results}. 

In the second experiment, we moved the torso slowly back and forth 
as well as rotating it. 
In the Velodyne driver, it combines several \emph{packets},
a small piece of point cloud, into a full scan of point cloud. Therefore, instant
jumps will cause motion distortion effect. However, it could be improved by motion 
compensation or applying a filter. The result is shown in Fig.~\ref{fig:LiDAR_results_moving}.

% Due to space limitations, these results are not presented. 
%\jwg{Remove dynamic data.}
% However, even if we have tried to move the torso slowly, 
% the ground in the testing field was bumpy and rough, which caused some instant ``jumps''
% in the \lidar\ measurement. In the Velodyne driver, it combines several \emph{packets},
% a small peice of point cloud, into a full scan of point cloud. Therefore, instant
% jumps will casuse motion distortion effect. However, it could be improved by motion 
% compensation or applying a filter.
% as shown in Fig. \red{FIG}.


\subsection{Discussion and Limitations}
% \bht{computation time vs more tags}
% lidar packets v
% motion compensation v
% limitation of dense range, v
% distance depends on devices v
% black-white <-> intensity v
% NN  v

In this work, we use a Velodyne 32-beam Ultra Pack.
% and we have checked the correct functioning of the proposed \lidart\ from $0.7$ m to $4$ m. 
The range limitation is because the \lidart\ has to be within a sufficiently \emph{dense} area of the \lidar's returns.
While a typical \lidars' vertical field of view (FOV) is $40^\circ$, only $20^\circ$ of the FOV
will have densely spaced beams. If a \lidart\ is not within the dense area of a \lidar, it will not
satisfy requirement of \eqref{eq:psi}, resulting in failed detections. As shown in Table 
\ref{tab:accuracy}, most of the computation time is spent on clustering edge points. Actual time spent on validation 
and other processes is relatively small. Thus, the number of  \lidarts\ in the FOV has little effect on computation time. 

% Additionally, if on-board computation power is a concern, simply limiting the \lidar\ range in
% the code should solve the problem, i.e. \lidars\ still work as they used to work.

As mentioned in Sec. \ref{sec:pose_acc}, a full scan (point cloud) from a Velodyne consists of several packets. Motion compensation is required if a robot moves
quickly. One solution is to transform each packet to the state estimation frame, correct the motion distortion effect, and transform the packet back to the sensor frame. For Cassie Blue, we send each individual packet to the IMU frame and use an invariant extended Kalman filter~\cite{barrau2016invariant,Hartley-RSS-18,hartley2018contact} to compensate
the motion distortion. The filter runs at $2~\mathrm{kHz}$ and compensates \lidar\ packets without any noticeable time delays. 

As summarized in Sec. \ref{sec:lidarVScamera}, the unstructured nature of a LiDAR's point cloud (irregular point distribution, missing returns, and varying spaces between returns) and the overall sparsity of points on a given marker made the decoding process challenging. In this paper, we proposed several means of meeting these challenges. One may suspect that ``deep learning'' could obviate many of the discrete steps we introduced. We gave this a try ourselves but we were unable to overcome issues such as rotation invariance of the network to tag orientating and domain adoption, which led us to employ the proposed remapping and weighted Gaussian voting to solve this problem. However, in the future we are interested in exploring the application of deep learning for this problem in more depth.




% \mgj{it's vague, explicitly mention what you mean rather than referring. Now the reader needs to go back and find 
% wht you mean before continuing which is annoying and interrupts the message.}
% \bh{Fixed}
% We have tried using naive classification (just classify wherever it is inside a grid) to decode;
% however, due to noisy and missing returns on the payload, it gives totally wrong
% results.
% \mgj{use formal English. Totally wrong result is totally informal! literally!}\bh{Fixed}

% \section{Discussion}
% lidar packets
% motion compensation
% mocap accuracy, 
% limitation of dense range,
% distance depends on devices
% black-white <-> intensity
% NN 


% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{LiDAR-Camera Calibration Evaluation}
% %In this section, we evaluate the three methods using both simulation data and experiments data. 
% In simulation, we randomly generate ground truth state $X_{\text{truth}}$
% and then apply noise to the ground truth state as our measurement as mentioned 
% in \eqref{eq:H_CL}. In experiments, measurement are $\hat{H}_{TL}$, 
% $\hat{H}_{TC}$. $\hat{H}_{CL}$ can then be computed from \eqref{eq:H_CL}.
% The error has been defined in \eqref{eq:calibration_acc}. The coordinate of a LiDAR, 
% a camera and tags are defined in Fig. \ref{fig:frame}.  

% In the InEKF and the mean method, we have options of doing an iterative solution or a batch solution. 
% Since in calibration, sensors are static and speed of filter is not concerned, 
% we chose incremental batch solution to help converge, where we incrementally
% accumulated a few synchronized pointcloud-image pairs and then incrementally solves as a
% batch solution as shown in \eqref{eq:correction_x} and \eqref{eq:correction_P}. 
% In Fig. \ref{fig:calibration_results}, 
% it shows the simulation results of calibration in three different
% methods:mean, iterative-batch InEKF, iterative-batch average mean and sample mean.
% The sample mean method works the best among these three methods. However, it has to
% collect the data all at once and then solves iteratively. 
% % In Fig. \ref{fig:exp_calibration}, it shows the result of calibration results of iterative-batch, 
% % iterative-batch average mean and sample mean.
% % \red{ADD more about accuracy after experiments}

% \begin{figure}[t]%
% \centering
% \subfloat[][Simulated results of calibration]{%
% \label{fig:sim_calibration}%
% \includegraphics[width=0.99\columnwidth]{sim_results.jpg}}\\
% \subfloat[][Experimental results of calibration]{%
% \label{fig:exp_calibration}%
% \includegraphics[width=0.4\columnwidth]{sim_results.jpg}}%
% \caption[]{\mgj{The legends are wrong. The iterative EKF has a specific meaning and is an estimation technique. What you do is Incremental InEKF vs Batch InEKF. Also too many words like ave mean batch are confusing. What's sample? I suggest only showing Incremental InEKF and Batch InEKF.}}%
% \label{fig:calibration_results}%
% \end{figure}





==> TagDesignShort.tex <==
\section{\add{Tag Design, \lidar Characteristics and Tag Detection}}
\label{sec:tag_design}
This section describes some essential points to consider when designing and using a
LiDAR-based tag system. In particular, this section addresses
how the unstructured point cloud from a LiDAR results in different considerations in
the selection of a marker versus those used with a camera. 

\subsection{LiDAR Point Clouds vs Camera Images}
\label{sec:lidarVScamera}
Pixel arrays (i.e., an image) from standard RGB-cameras of different resolutions are
very structured, with the pixels arranged in a uniform (planar) grid, and each image
having a fixed number of data points. A LiDAR returns $(x,y,z)$ coordinates of
an object relative to a fixed frame in the device as well as the intensity, which
relies on the reflectivity/material of the object. Some \lidars also provide beam
numbers. The resulting 3D point clouds are typically referred to as ``unstructured''
because: 
\begin{itemize}
\item The number of returned points varies for each scan and for each beam. In
    particular, LiDAR returns are not uniformly distributed in angle or
    distance\footnote{Some \lidars have different ring density at different
    elevation angles. For example, \velodyne has dense ring density between
    $-5^\circ$ and $3^\circ$, and has sparse ring density from $-25^\circ$ to
    $-5^\circ$ and from $3^\circ$ to $15^\circ$~\cite{velodyneUltraPuck}.
    Therefore, in a sparse region, a target may be only partially 
    illuminated/observed.}.
\item  As shown in Fig.~\ref{fig:irregular}, high contrast between adjacent regions of a
    target's surface can result in missing returns and in varying spaces between
    returns. 
\item When used outdoors, the number of returned points is also
    influenced by environmental factors such as weather, especially temperature.
\end{itemize}
Consequently, as opposed to an image, there is no fixed geometric relationship
between the index numbers of returns from two different beams in a multi-beam LiDAR.
A further difference is the density of the collected data; currently, basic cameras
provide many more data points for a given surface size at a given distance than even
high-end \lidarsN. These summarized differences have an impact on how one approaches
the design of a LiDAR-based tag system vs a camera-based tag system. 

% The unstructured nature of the point clouds vs camera images has implciations for the 
% The well-known fiducial tag systems \cite{???} exploit this structure in their algorithms. 

% LiDAR has accurate distance, hence using distance for edge detection of the tag becomes interesting.

% .

% Density of measured values on a tag will be much lower with LiDAR than with today's cameras



% For a 15 cm x 15 cm "payload" at a distance of 2 m -----give idea of the number of returns one can expect vs 
% a typical camera's number of pixels. 11,642/100.

% Number of points affected by temperature.

% Because pixels are in a uniform grid, 

% %Unaffected by lighting<-----red herring 

% LiDARs are different from cameras. Once selected a resolution, 
% cameras have fixed number of pixels for all the images. 
% % A scan of point cloud from LiDAR is usually expressed in beam. 
% Given a same beam number, 
% we still have much different amount of points in different LiDAR
% such as Velodyne HDL-32E and Velodyne ULTRA PUCK \red{CITE?}. Point clouds from 
% the same LiDAR do not have the same amount of points in each scan. 
% Moreover, it also depends on the weather: if 
% the weather is warm/hot, the size of the point clouds are smaller; larger if cold. 
% Thus, it is critical to analyze the LiDAR device Sec. \ref{sec:analysis} first every time it starts.

% \begin{figure}[t]%
%     \centering
%     \includegraphics[width=1\columnwidth]{irregular_points.png}%
%     \caption[]{This figure illustrates the unstructured nature of a LiDAR-point-cloud return (top) for a planar surface with black and white squares (bottom). The returns are more irregular at the square boundaries. Red circles indicate missing
%         returns and green bars highlight larger gaps between returned points. \jwg{We need the true image below and the LiDAR return above it.}
% }%
% \end{figure}

\begin{figure}[t]%
\centering
%\label{fig:tag_explain}%
\subfloat{%
\includegraphics[height=0.4\columnwidth]{IrregularPoints.png}}%
\subfloat{%
\hspace{8pt}
%\label{fig:tag_explain}%
\includegraphics[trim=0 0 0 0,clip, height=0.4\columnwidth]{LiDARTagImg.png}}%
\caption[]{This figure illustrates the unstructured nature of a LiDAR-point-cloud
return (left) for a planar surface with black and white squares (right). On the left,
the black and white dots are lower reflectivity and higher reflectivity, respectively.
The sparse region of the \lidar is indicated in light yellow and the dense region is
marked in light blue. The returns are more irregular at the black-white transitions.
Red circles indicate missing returns and green bars highlight larger gaps between
returned points.
}%
\label{fig:irregular}%
\end{figure}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Tag Placement and Design }
\label{sec:selection}
As mentioned in Sec. \ref{sec:lidarVScamera}, a return from a typical LiDAR
consists of an $(x,y,z)$ measurement, an intensity value $i$, and a
beam number (often called ring number, $r$). In this
paper, we propose exploiting the
relative accuracy of a LiDAR's distance measurement to determine ``features'' when
seeking to isolate a LiDARTag in a 3D point cloud (see Sec.~\ref{sec:Detection}) and
associating the isolated \lidart points with a
continuous function to decode the marker's payload (see Sec.~\ref{sec:Decoding}).
% \dels{It is further proposed to use \emph{intensity} to isolate and decode the tag's
% ID.}


\subsubsection{Tag design}
A LiDARTag is assumed to consist of a planar fiducial marker rigidly attached to
    a 3D object, as shown in Fig.~\ref{fig:3dtag}. In particular, the marker shows
different intensity values when illuminated by a \lidarN. As indicated in
    Sec.~\ref{sec:lidarVScamera}, intensity relies on an object's reflectivity and
    material. Most types of fiducial markers for camera-based systems could be adapted for use in LiDAR-based systems as long as
    the payload is composed of differing reflectivities and is placed inside the
 region highlighted in yellow in Fig.~\ref{fig:tag_explain}. Figure~\ref{fig:MarkerExample} shows
    an example of an \atag used as a \lidartN. Because fiducial markers are usually
    printed from a printer, however, markers with two colors such as \atag 1-3
    \cite{olson2011apriltag, wang2016apriltag, krogiusflexible},
    ARTag~\cite{fiala2005artag, fiala2005comparing},
    InterSense~\cite{naimark2002circular}, CyberCode~\cite{rekimoto2000cybercode}, or
    CALTag~\cite{atcheson2010caltag} can be most easily adapted for use in our \lidart system, while
Cho et.al~\cite{cho1998multi} cannot. 


% \del{The fiducial marker is assumed to consist of a clearly delineated black and white
% boundary surrounding a payload consisting of a black and white pattern. The intensity
% difference of the LiDAR returns for the black and white boundary will be used in
% secondary edge detection, as described later in Sec.~\ref{sec:validation.}}
% 
% 
% \del{With these \emph{assumptions}, tag families such as AprilTag 1-3
% \cite{olson2011apriltag, wang2016apriltag, krogiusflexible},
% ARTag~\cite{fiala2005artag, fiala2005comparing}, or
% InterSense~\cite{naimark2002circular} can be adapted for use in our LiDARTag system,
% but not those in CyberCode~\cite{rekimoto2000cybercode}, Cho
% et.al~\cite{cho1998multi} nor CALTag~\cite{atcheson2010caltag}.}

% These are summarized in Fig.~\ref{fig:tag_family}. 

% \begin{figure}[th!]%
% \centering
% \subfloat{%
% \includegraphics[width=0.45\columnwidth]{lighting2.jpg}}%
% \hspace{10pt}%
% \subfloat{%
% \label{fig:toTag}%
% \includegraphics[width=0.45\columnwidth]{lighting1.jpg}}\\
% \subfloat{%1
% \label{fig:toLiDAR}%
% \includegraphics[width=0.46\columnwidth]{lighting3.jpg}}
% \hspace{12pt}%
% \subfloat{%
% \label{fig:torso}%
% \includegraphics[trim=0 10 0 0,clip,width=0.42\columnwidth]{torso.jpg}}%
% \caption[]{Point clouds from LiDARs are robust to lighting. LiDARTags can be
% detected in these three extreme cases: a completely dark environment, shining a 
% strong spotlight onto a LiDARTag, pointing a strong spotlight at a LiDAR sensor. 
% Bottom right shows the Velodyne 32-beam Ultra Puck in
% red, an Intel RealSense in green, and markers for a motion capture system in blue.}%
% \label{fig:environment}%
% \end{figure}

\begin{figure}[t]%
\centering
\subfloat[]{%
    \label{fig:3dtag}%
    \includegraphics[width=0.4\columnwidth]{LiDARTagSideView.png}}%
\hspace{10pt}%
\subfloat[]{%
    \label{fig:tag_explain}%
    \includegraphics[width=0.5\columnwidth]{LiDARTagFrontView.png}}\\
\subfloat[]{%
    \label{fig:MarkerExample}%
    \includegraphics[width=0.4\columnwidth]{MarkerExample.png}}%
\hspace{10pt}%
\subfloat[]{%
\label{fig:torso}%
\includegraphics[trim=0 10 0 0,clip,width=0.45\columnwidth]{torso.png}}%
\caption[]{\subref{fig:3dtag} illustrates a \lidart consisting of two parts: 
a 3D object with a rigidly attached, planar fiducial marker where $t$ and $h$ are the
marker size and height of the object respectively. \subref{fig:tag_explain} shows the
marker should be placed inside the yellow region and \subref{fig:MarkerExample}
illustrates an example of \atag being used as a \lidartN. \subref{fig:torso}
is the sensor setup consisting of a \lidarN, a camera and several motion capture
markers.
}%
\squeezeup
\label{fig:LiDARTag}%
\end{figure}



\begin{figure*}[t!]
    \includegraphics[width=\linewidth]{Pipelinev3.png}
    \caption{
        The system contains three parts: tag detection, pose estimation, and tag
        decoding. The detection step takes an entire \lidar scan (up to 120,000
        points from a \velodyneN) and outputs collections of likely payload points of
        the \lidartsN. Next, a tag's optimal pose minimizes the $L_1$-inspired cost
        in \eqref{eq:JKHcost}, though the rotation of the tag about a normal vector
        to the tag may be off by $\pm 90^\circ$ or $180^\circ$ and will be resolved in
        the decoding process. Later, a 3D-shape point cloud is constructed based on
        the intensity of \lidartN's returns, and a continuous function is built in a
        RKHS. The final decoding process is to compute
        the inner product of the continuous functions in a pre-computed function
    dictionary and the rotation ambiguity about the normal is determined.}
     
    \label{fig:pipline}
    \squeezeup
\end{figure*}

% \begin{figure}[t]%
% \centering
% \subfloat[]{%
% \label{fig:3dtag}%
% \includegraphics[width=0.25\columnwidth]{3dlidartag.png}}%
% \hspace{1pt}%
% \subfloat[]{%
% \label{fig:tag_explain}%
% \includegraphics[trim=0 18 0 0,clip,width=0.32\columnwidth]{tag_explain.png}}%
% \hspace{1pt}%
% \subfloat[]{%
% \label{fig:torso}%
% \includegraphics[trim=0 10 0 0,clip,width=0.4\columnwidth]{torso.png}}%
% \caption[]{The left illustrates a possible \lidart\ consisting of two parts: 
% a freestanding 3D object with a rigidly attached, planar fiducial marker. 
% On the middle, a fiducial marker is outlined in red and the payload is outlined in green. 
% In this particular marker, $d$ is $4$, the number of squares in a row.}%
% \squeezeup
% \label{fig:LiDARTag}%
% \end{figure}
%\jwg{Why not have a different number of rows and columns to aid in determining orientation?}

For this initial study, we employ \atagN3 as our fiducial markers.
Furthermore, within the \atagN3 family of markers, we select tag16h6c5,
 that is, a tag encoding 16 bits (i.e., 16 black or white squares), with a
minimum Hamming distance of 6, and a complexity of 5. The Hamming distance measures
the minimum number of bit changes (e.g., bit errors) required to transform one string
of bits into the other. For example, the length-7 strings $``1011111"$ and
$``1001011"$ have a Hamming distance of 2, whereas $``1011111"$ and $``1001010"$ have
a Hamming distance of 3. The significance is that a lexicode with a minimum Hamming
distance $h$ can detect $h/2$ bit errors and correct up to $\floor{(h-1)/2}$ bit
errors~\cite{trachtenbert1996computational}. The complexity of an \atag is defined
as the number of rectangles required to generate the tag’s 2D pattern. For example, a
solid pattern requires just one rectangle, whereas, a white-black-white stripe would
need two rectangles (first draw a large white rectangle; then draw a smaller black
rectangle). For further details, we refer the reader to the coding discussion
in Olson~\cite{olson2011apriltag}.


\begin{remark}
One may argue that other members of the \atagsN3 family, such as tag49h15c15,
tag36h11c10, tag36h10c10, and tag25h10c8, would be more appropriate. For example,
including more bits tends to increase the number of distinct tags in a family, while
a larger Hamming distance reduces false positives. However, for tags of the same
physical size and the same distance from the sensor, more bits means fewer returns
per square and a higher error rate for individual squares.
\end{remark}

\subsubsection{Tag placement}
In Fig.~\ref{fig:3dtag}, let $t$ be the tag size and $h$ be the thickness of the 3D
object. The 3D object is assumed to have $t\sqrt{2}/4$ clearance around it, and
the first \lidar ring hitting at a \lidart is above $3/4$ of the \lidartN, see
Sec.~\ref{sec:clustering}. In particular, the fiducial marker can be
attached to a wall as long as the condition, $h>t\sqrt{2}/4$, in Fig.~\ref{fig:3dtag} is met. Finally, it is not recommended to orient the marker
like a square due to the quantization error inherited in \lidar sensors, see
\cite[Sec. II]{huang2019improvements}.


\subsection{Tag Detection}
\label{sec:Detection}
\add{
Tag detection and validation are criteria but easily replaceable by other methods,
such as deep-learning-based detector. Due to the page limit of the paper, only an
overview of tag detection and validation processes is provided. For more detail of
each step, we refer readers to the full version of the paper on arXiv~\bh{full
version}. 
}

\add{
    The overall pipeline is shown in Fig.~\ref{fig:pipline}. Inspired by the point
    selection method in LeGO-LOAM~\cite{legoloam2018}, an edge point is defined as
    discontinuities in distance. A point is defined as a feature if it is an edge
    point, and its consecutive $n$ points are not edge points (similar to plane
    features in LeGO-LOAM). 
}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{LiDAR Characteristics Analysis}
% \label{sec:analysis}
% \jwg{Not edited by me. Maybe it's a detail that can be skipped?} \mgj{I agree. The subsection is unnecessary and can be removed. If there is one or two sentences you'd like to include add it to the discussion or where you explain the algorithm as a remark.}
% As mentioned in Sec.~\ref{sec:lidarVScamera}, a scan of point clouds 
% from a Velodyne 32-beam Ultra Pack is up to 1.3 million returned points. 
% However, actual returned points on a payload are sparse. 
% A scan of point clouds from a LiDAR device is usually made of many beams. For example, a scan of 
% point clouds from Velodyne 32-beam is made of the 32 beams of returned points.
% Inconsistency and irregularity mentioned in Sec.~\ref{sec:lidarVScamera} vastly 
% challenge the robustness of a system. 
% Therefore, let the detector, described in Sec.~\ref{sec:detection}, observe the 
% characteristics of this specific LiDAR at this moment, at this weather is essential,
% particularly how many points in a scan, how many points on each beam.
% Thus, at the beginning of the algorithm, we create two tables: a point table that records how
% many points on each beam and another table summarizes the average, maximum, minimum size of 
% each scan of of point clouds. Note, this only needs to be done one time 
% at the beginning of the algorithm.


==> defines_.tex <==
\usepackage{url}
\usepackage[usenames,dvipsnames,svgnames,table, xcdraw]{xcolor}
\usepackage{multicol}
\usepackage{natbib}
\usepackage{graphicx}
\usepackage{caption}
\captionsetup{size=footnotesize,
    %justification=centering, %% not needed
    %skip=5pt, position = bottom}
    position = bottom}
    
\graphicspath{
    {graphics/}
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \usepackage{amsmath,amssymb,enumerate}
% \let\proof\relax 
% \let\endproof\relax
% \usepackage{amsthm}
\usepackage{amsmath,amssymb,thmtools,enumerate}
\usepackage[noadjust]{cite}
\usepackage{setspace}
\usepackage{booktabs}
\usepackage{stmaryrd}
\usepackage[colorlinks=true,pdfpagemode=UseNone,citecolor=black,linkcolor=black,urlcolor=BrickRed]{hyperref}
% \usepackage{mathtools}
\usepackage{algorithm, algorithmicx, algpseudocode}
\renewcommand{\algorithmiccomment}[1]{\hfill$\triangleright$~\textcolor{Gray}{#1}}
% \usepackage{blindtext}
% \usepackage{gensymb}
\usepackage{xparse}
% \usepackage{lipsum}
%\usepackage{subcaption}
\usepackage{soul} 
% \usepackage{mathrsfs}
% \usepackage[mathscr]{euscript}
% \usepackage{times}
% \usepackage{cleveref}
% \usepackage{cite} % to group references
\usepackage[caption=false,font=footnotesize]{subfig}
% \usepackage{amsfonts}
% \usepackage[utf8]{inputenc}
% \usepackage[T1]{fontenc}
% \usepackage{textcomp}
% \usepackage{balance}
% \usepackage{calligra}
\usepackage{multirow}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5
% \newtheorem{fact}{Fact}

\def\realnumbers{\mathbb{R}}
\DeclareMathOperator*{\argmin}{arg\,min}
% \DeclareMathOperator*{\minimize}{minimize}
% \newcommand\scalemath[2]{\scalebox{#1}{\mbox{\ensuremath{\displaystyle #2}}}}
% \renewcommand{\thefigure}{\arabic{figure}}


\newcommand{\hilight}[1]{\colorbox{yellow}{#1}} % to use: \hl{this is some highlighted text}
\newcommand{\red}[1]{{\textcolor{red}{#1}}}
\newcommand{\blue}[1]{{\textcolor{blue}{#1}}}
\newcommand{\rha}[1]{[{\textbf{\textcolor{orange}{Ross: #1}}}]}
\newcommand{\jwg}[1]{[{\textbf{\textcolor{red}{JWG: #1}}}]}
\newcommand{\mgj}[1]{[{\textbf{\textcolor{teal}{Maani: #1}}}]}
\newcommand{\jkh}[1]{[{\textbf{\textcolor{blue}{Bruce: #1}}}]}
\newcommand{\bh}[1]{[{\textbf{\textcolor{blue}{Bruce: #1}}}]}
\newcommand{\bht}[1]{[{\textbf{\textcolor{note}{Bruce: (TODO) #1}}}]}
\newcommand{\bhd}[1]{[{\textbf{\textcolor{blue}{Bruce: Done, please check#1}}}]}
\definecolor{note}{rgb}{0.3,0.7,0.25}
\definecolor{rephase}{rgb}{0.15,0.7,0.15}
\definecolor{bag}{rgb}{0.6,0.6,0.2}



\newcommand{\lidar}{LiDAR}
\newcommand{\lidars}{LiDARs}
\newcommand{\lidart}{LiDARTag}
\newcommand{\lidarts}{LiDARTags}
\newcommand{\atag}{AprilTag}
\newcommand{\atags}{AprilTags}


% \newcommand{\bigO}[1]{\Ocal(#1)} % Big O
% \newcommand{\EV}[1]{\mathbb{E}[#1]} % Expected Value
% \newcommand{\Var}[1]{\mathbb{V}[#1]} % Variance
% \newcommand{\Covariance}[1]{\mathbf{Cov}[#1]} % Covariance
\newcommand{\floor}[1]{\lfloor #1 \rfloor}

% \newcommand{\diag}{\mathop{\mathrm{diag}}}
% \newcommand{\m}{\mathop{\mathrm{m}}}
% \newcommand{\rad}{\mathop{\mathrm{rad}}}
% \newcommand{\dBm}{\mathop{\mathrm{dBm}}}
% \newcommand{\Hz}{\mathop{\mathrm{Hz}}}
% \newcommand{\GHz}{\mathop{\mathrm{GHz}}}
% \newcommand{\MHz}{\mathop{\mathrm{MHz}}}

% \newcommand{\Acal}{\mathcal{A}}
% \newcommand{\Bcal}{\mathcal{B}}
% \newcommand{\Ccal}{\mathcal{C}}
% \newcommand{\Dcal}{\mathcal{D}}
% \newcommand{\dcal}{\text{\calligra d }}
% \newcommand{\ccal}{\text{\calligra c }}
% \newcommand{\Fcal}{\mathcal{F}}
% \newcommand{\GPcal}{\mathcal{GP}}
% \newcommand{\Hcal}{\mathcal{H}}
% \newcommand{\Ical}{\mathcal{I}}
% \newcommand{\Kcal}{\mathcal{K}}
% \newcommand{\Lcal}{\mathcal{L}}
% \newcommand{\Mcal}{\mathcal{M}}
\newcommand{\Ncal}{\mathcal{N}}
% \newcommand{\Ocal}{\mathcal{O}}
% \newcommand{\Scal}{\mathcal{S}}
% \newcommand{\Tcal}{\mathcal{T}}
% \newcommand{\Xcal}{\mathcal{X}}
% \newcommand{\Ycal}{\mathcal{Y}}
% \newcommand{\Zcal}{\mathcal{Z}}

% \newcommand{\Exp}{\mathrm{Exp}}
% \newcommand{\Log}{\mathrm{Log}}
% \newcommand{\Jr}{\mathrm{J_r}}
\newcommand{\transpose}{\mathsf{T}}
% \newcommand{\SO}{\mathrm{SO}}
% \newcommand{\SE}{\mathrm{SE}}
% \newcommand{\GL}{\mathrm{GL}}
% \newcommand\inv[1]{#1\raisebox{1.15ex}{$\scriptscriptstyle-\!1$}}

% \newcommand{\vecToSkew}{\wedge}
% \newcommand{\skewToVec}{\hat}
% \DeclareDocumentCommand{\vectorToSkew}{ O{} }{\left(#1\right)_\times}

\DeclareDocumentCommand{\vector}{ O{} }{\mathrm{vec}(#1)}
\DeclareDocumentCommand{\zeros}{ O{} }{\textbf{0}_{#1}}
\DeclareDocumentCommand{\X}{ O{} O{} }{\textbf{X}_{#1}^{#2}}
% \DeclareDocumentCommand{\XE}{ O{} O{} }{\hat{\textbf{X}}_{#1}^{#2}}
% \DeclareDocumentCommand{\B}{ O{} O{} }{\textbf{B}_{#1}^{#2}}
% \DeclareDocumentCommand{\H}{ O{} O{} }{\textbf{H}_{#1}^{#2}}
% \DeclareDocumentCommand{\L}{ O{} O{} }{\textbf{L}_{#1}^{#2}}
% \DeclareDocumentCommand{\M}{ O{} O{} }{\textbf{M}_{#1}^{#2}}
% \DeclareDocumentCommand{\m}{ O{} O{} }{\textbf{m}_{#1}^{#2}}
% \DeclareDocumentCommand{\S}{ O{} O{} }{\textbf{S}_{#1}^{#2}}
\DeclareDocumentCommand{\P}{ O{} O{} }{\textbf{P}_{#1}^{#2}}
% \DeclareDocumentCommand{\Q}{ O{} O{} }{\textbf{Q}_{#1}^{#2}}
% \DeclareDocumentCommand{\J}{ O{} O{} }{\textbf{J}_{#1}^{#2}}
% \DeclareDocumentCommand{\R}{ O{} O{} }{\textbf{R}_{#1}^{#2}}
% \DeclareDocumentCommand{\RE}{ O{} O{} }{\hat{\textbf{R}}_{#1}^{#2}}
% \DeclareDocumentCommand{\Q}{ O{} O{} }{\textbf{Q}_{#1}^{#2}}
% \DeclareDocumentCommand{\T}{ O{} O{} }{\textbf{T}_{#1}^{#2}}
% \DeclareDocumentCommand{\L}{ O{} O{} }{\textbf{L}_{#1}^{#2}}
% \DeclareDocumentCommand{\K}{ O{} O{} }{\textbf{K}_{#1}^{#2}}
\DeclareDocumentCommand{\V}{ O{} O{} }{\textbf{V}_{#1}^{#2}}
% \DeclareDocumentCommand{\N}{ O{} O{} }{\textbf{N}_{#1}^{#2}}
\DeclareDocumentCommand{\Y}{ O{} O{} }{\textbf{Y}_{#1}^{#2}}
% \DeclareDocumentCommand{\Z}{ O{} O{} }{\textbf{Z}_{#1}^{#2}}
% \DeclareDocumentCommand{\F}{ O{} O{} }{\textbf{F}_{#1}^{#2}}
% \DeclareDocumentCommand{\G}{ O{} O{} }{\textbf{G}_{#1}^{#2}}
% \DeclareDocumentCommand{\A}{ O{} O{} }{\textbf{A}_{#1}^{#2}}
% \DeclareDocumentCommand{\TH}{ O{} O{} }{\boldsymbol{\Theta}_{#1}^{#2}}
% \DeclareDocumentCommand{\w}{ O{} O{} }{\textbf{w}_{#1}^{#2}}
% \DeclareDocumentCommand{\x}{ O{} O{} }{\textbf{x}_{#1}^{#2}}
% \DeclareDocumentCommand{\y}{ O{} O{} }{\textbf{y}_{#1}^{#2}}
% \DeclareDocumentCommand{\e}{ O{} O{} }{\textbf{e}_{#1}^{#2}}
% \DeclareDocumentCommand{\c}{ O{} O{} }{\textbf{c}_{#1}^{#2}}
% \DeclareDocumentCommand{\C}{ O{} O{} }{\textbf{C}_{#1}^{#2}}
% \DeclareDocumentCommand{\CM}{ O{} O{} }{\tilde{\textbf{C}}_{#1}^{#2}}
% \DeclareDocumentCommand{\RM}{ O{} O{} }{\tilde{\textbf{R}}_{#1}^{#2}}
% \DeclareDocumentCommand{\I}{ O{} O{} }{\textbf{I}_{#1}^{#2}}
% \DeclareDocumentCommand{\O}{ O{} O{} }{\textbf{O}_{#1}^{#2}}
% \DeclareDocumentCommand{\r}{ O{} O{} }{\textbf{r}_{#1}^{#2}}
% \DeclareDocumentCommand{\t}{ O{} O{} }{\textbf{t}_{#1}^{#2}}
% \DeclareDocumentCommand{\k}{ O{} O{} }{\textbf{k}_{#1}^{#2}}
% \DeclareDocumentCommand{\u}{ O{} O{} }{\textbf{u}_{#1}^{#2}}
\DeclareDocumentCommand{\U}{ O{} O{} }{\textbf{U}_{#1}^{#2}}
% \DeclareDocumentCommand{\d}{ O{} O{} }{\textbf{d}_{#1}^{#2}}
% \DeclareDocumentCommand{\dE}{ O{} O{} }{\hat{\textbf{d}}_{#1}^{#2}}
% \DeclareDocumentCommand{\b}{ O{} O{} }{\textbf{b}_{#1}^{#2}}
% \DeclareDocumentCommand{\a}{ O{} O{} }{\textbf{a}_{#1}^{#2}}
% \DeclareDocumentCommand{\g}{ O{} O{} }{\textbf{g}_{#1}^{#2}}
% \DeclareDocumentCommand{\f}{ O{} O{} }{\textbf{f}_{#1}^{#2}}
% \DeclareDocumentCommand{\dM}{ O{} O{} }{\tilde{\textbf{d}}_{#1}^{#2}}
% \DeclareDocumentCommand{\params}{ O{} O{} }{\boldsymbol{\theta}_{#1}^{#2}}
% \DeclareDocumentCommand{\paramsE}{ O{} O{} }{\hat{\boldsymbol{\theta}}_{#1}^{#2}}
% \DeclareDocumentCommand{\paramError}{ O{} O{} }{\boldsymbol{\zeta}_{#1}^{#2}}
% \DeclareDocumentCommand{\gyroscopeBias}{ O{} }{\textbf{b}_{#1}^{g}}
% \DeclareDocumentCommand{\gyroscopeBiasE}{ O{} }{\hat{\textbf{b}}_{#1}^{g}}
% \DeclareDocumentCommand{\accelerometerBias}{ O{} }{\textbf{b}_{#1}^{a}}
% \DeclareDocumentCommand{\accelerometerBiasE}{ O{} }{\hat{\textbf{b}}_{#1}^{a}}
% \DeclareDocumentCommand{\position}{ O{} O{} }{{}_\text{#2}\textbf{p}_{\text{#1}}}
% \DeclareDocumentCommand{\positionDot}{ O{} O{} }{{}_\text{#2}\dot{\textbf{p}}_{\text{#1}}}
% \DeclareDocumentCommand{\linearVelocity}{ O{} O{} }{{}_\text{#2}\textbf{v}_{\text{#1}}}
% \DeclareDocumentCommand{\linearVelocityM}{ O{} O{} }{{}_\text{#2}\tilde{\textbf{v}}_{\text{#1}}}
% \DeclareDocumentCommand{\orientation}{ O{} }{\textbf{R}_{\text{#1}}}
% \DeclareDocumentCommand{\orientationDot}{ O{} }{\dot{\textbf{R}}_{\text{#1}}}
% \DeclareDocumentCommand{\homogeneous}{ O{} O{} }{{}_\text{#2}\boldsymbol{\H}_{\text{#1}}}
% \DeclareDocumentCommand{\homogeneousDot}{ O{} }{\dot{\textbf{H}}_{\text{#1}}}
% \DeclareDocumentCommand{\Jacobian}{ O{} O{} }{{}_\text{#2}\boldsymbol{\J}_{\text{#1}}}
% \DeclareDocumentCommand{\inputs}{ O{} O{} }{{}_\text{#2}\boldsymbol{\u}_{\text{#1}}}
% \DeclareDocumentCommand{\inputsM}{ O{} O{} }{{}_\text{#2}\tilde{\boldsymbol{\u}}_{\text{#1}}}
% \DeclareDocumentCommand{\angularVelocity}{ O{} O{} }{{}_\text{#2}\boldsymbol{\omega}_{\text{#1}}}
% \DeclareDocumentCommand{\angularVelocityM}{ O{} O{} }{{}_\text{#2}\tilde{\boldsymbol{\omega}}_{\text{#1}}}
% \DeclareDocumentCommand{\acceleration}{ O{} O{} }{{}_\text{#2}\textbf{a}_{\text{#1}}}
% \DeclareDocumentCommand{\accelerationM}{ O{} O{} }{{}_\text{#2}\tilde{\textbf{a}}_{\text{#1}}}
% \DeclareDocumentCommand{\p}{ O{} O{} }{\textbf{p}_{#1}^{#2}}
% \DeclareDocumentCommand{\pE}{ O{} O{} }{\hat{\textbf{p}}_{#1}^{#2}}
% \DeclareDocumentCommand{\pM}{ O{} O{} }{\tilde{\textbf{p}}_{#1}^{#2}}
% \DeclareDocumentCommand{\v}{ O{} O{} }{\textbf{v}_{#1}^{#2}}
% \DeclareDocumentCommand{\vE}{ O{} O{} }{\hat{\textbf{v}}_{#1}^{#2}}
% \DeclareDocumentCommand{\w}{ O{} O{} }{\boldsymbol{\omega}_{#1}^{#2}}
% \DeclareDocumentCommand{\wM}{ O{} O{} }{\tilde{\boldsymbol{\omega}}_{#1}^{#2}}
% \DeclareDocumentCommand{\angleTheta}{ O{} O{} }{\boldsymbol{\theta}_{#1}^{#2}}
% \DeclareDocumentCommand{\anglePhi}{ O{} O{} }{\boldsymbol{\phi}_{#1}^{#2}}
% \DeclareDocumentCommand{\encoders}{ O{} O{} }{\boldsymbol{\alpha}_{#1}^{#2}}
% \DeclareDocumentCommand{\encodersM}{ O{} O{} }{\tilde{\boldsymbol{\alpha}}_{#1}^{#2}}
% \DeclareDocumentCommand{\offsets}{ O{} O{} }{\boldsymbol{\epsilon}_{#1}^{#2}}
% \DeclareDocumentCommand{\Cov}{ O{} O{} }{\boldsymbol{\Sigma}_{#1}^{#2}}
% \DeclareDocumentCommand{\Axis}{ O{} O{} }{\textnormal{Axis}_{#1}^{#2}}
% \DeclareDocumentCommand{\using}{ O{} O{} }{\stackrel{\mathmakebox[\widthof{=}]{\text{eq.} (#1)}}{#2} \enspace}
% \DeclareDocumentCommand{\Adjoint}{ O{} }{\mathrm{Ad}_{#1}}
% \DeclareDocumentCommand{\vectorToAlgebra}{ O{} }{\mathscr{L}_\mathfrak{g}\left(#1\right)}
% \DeclareDocumentCommand{\groupError}{ O{} O{} }{\boldsymbol{\eta}_{#1}^{#2}}
% % \DeclareDocumentCommand{\tangentError}{ O{} O{} }{\boldsymbol{\xi}_{#1}^{#2}}
% \DeclareDocumentCommand{\twist}{ O{} O{} }{\boldsymbol{\xi}_{#1}^{#2}}
% \DeclareDocumentCommand{\twistM}{ O{} O{} }{\tilde{\boldsymbol{\xi}}_{#1}^{#2}}

% \DeclareDocumentCommand{\JFK}{ O{} }{\textbf{J}^{\hspace{-0.75mm}\FK}_{#1}}

% \DeclareDocumentCommand{\JFKswitch}{ O{} }{\textbf{J}^{\hspace{-0.75mm}\FKswitch}_{#1}}

\newcommand{\squeezeup}{\vspace{-4mm}}

% \makeatletter
% \newcommand{\mathleft}{\@fleqntrue\@mathmargin0pt}
% \newcommand{\mathcenter}{\@fleqnfalse}
% \makeatother


==> tables.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Pose accuracy
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[]
\center
\caption{
This table shows the decoding accuracy of the RKHS method and pose accuracy of the
$L_1$-inspired fitting method. The ground truth is provided by a motion capture
system with 30 motion capture cameras. The distance is in meters. The translation is in
millimeters and rotation is the Geodesic metric in degrees.
}
\label{tab:PoseAccuracy}
\resizebox{2\columnwidth}{!}{%
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
\hline
\multicolumn{5}{|c|}{\textbf{Face-on to LiDAR}}                                    & \multicolumn{5}{c|}{\textbf{Rotated at 45 degrees}}                        \\ \hline
Distance         & No. Scans & No. Wrong ID   & Translation Error & Rotation Error & Distance & No. Scans & No. Wrong ID   & Translation Error & Rotation Error \\ \hline
2.15          & 73.00 & 0        & 14.03 & 0.44  & 2.13  & 74.00  & 0        & 0.27  & 0.05  \\ \hline
4.29          & 72.00 & 0        & 10.13 & 0.67  & 3.95  & 134.00 & 0        & 0.52  & 0.34  \\ \hline
5.90          & 81.00 & 0        & 16.23 & 0.44  & 5.93  & 137.00 & 0        & 0.36  & 0.05  \\ \hline
7.97          & 78.00 & 0        & 1.32  & 0.21  & 7.92  & 126.00 & 0        & 0.26  & 0.32  \\ \hline
10.12         & 87.00 & 0        & 1.64  & 0.40  & 10.38 & 130    & 0        & 4.91  & 1.03  \\ \hline
12.14         & 69.00 & 0        & 2.07  & 0.36  & 12.12 & 71.00  & 0        & 5.78  & 0.39  \\ \hline
13.87         & 35.00 & 1        & 2.81  & 10.48 & 14.08 & 49.00  & 2        & 1.98  & 15.92 \\ \hline
\textbf{Summary} & No. Scans & Wrong ID Ratio & Translation Error & Rotation Error & Summary  & No. Scans & Wrong ID Ratio & Translation Error & Rotation Error \\ \hline
\textbf{mean} & 70    & 0.202 \% & 6.891 & 2.149 & mean  & 103    & 0.276 \% & 1.744 & 2.586 \\ \hline
\textbf{std}  & 16.88 & --       & 6.418 & 4.577 & std   & 37.25  & --       & 2.076 & 5.888 \\ \hline
\end{tabular}
}
\end{table*}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Timing each step 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[]
\center
\caption{
    This table averages all the datasets we collected and
    describes computation time of each step for indoors and outdoors.
}
\label{tab:timing}
\resizebox{0.9\columnwidth}{!}{%
\begin{tabular}{|c|c|c|c|}
\hline
\multicolumn{4}{|c|}{\textbf{Outdoor}}                                     \\ \hline
No. Points & No. Features          & No. Clusters      & Total Computation \\ \hline
51717        & 2179          & 271            & 114.86 Hz         \\ \hline
PoI Clustering  & Fill In Clusters & Point Check       & Plane Fitting     \\ \hline
2.63 ms         & 0.3 ms           & 0.00 ms           & 0.27  ms          \\ \hline
Line Fitting    & PCA              & Pose Optimization & Tag Decoding      \\ \hline
0.01 ms         & 0.03 ms          & 0.48 ms           & 3.34 ms           \\ \hline
\multicolumn{4}{|c|}{\textbf{Indoor}}                                      \\ \hline
No. Point Cloud & No. Features          & No. Clusters      & Total Computation \\ \hline
54277        & 1820          & 225            & 102.41 Hz         \\ \hline
PoI Clustering  & Fill In Clusters & Point Check       & Plane Fitting     \\ \hline
3.28 ms         & 0.22 ms          & 0.00 ms           & 0.15 ms           \\ \hline
Line Fitting    & PCA              & Pose Optimization & Tag Decoding      \\ \hline
0.01 ms         & 0.01 ms          & 0.42 ms           & 2.47 ms           \\ \hline
\end{tabular}
}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Clusters rejected by each step 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[]
\center
\caption{
    This table takes into account all the data we collected and shows numbers of
    rejected clusters in each step in different scenes. Additionally, we also report
false positive rejection for Cartographer and H3D dataset.
}
\label{tab:remainingcClusters}
\resizebox{0.9\columnwidth}{!}{%
    \begin{tabular}{|c|c|c|}
\hline
\multicolumn{3}{|c|}{\textbf{Outdoor}}                           \\ \hline
No. Min. Return     & No. Max. Return     & No. Plane Fitting    \\ \hline
247.72              & 3.41                & 14.71                \\ \hline
No. Boundary Points & No. Pose Estimation & No. Decoding Failure \\ \hline
4.10                & 0.48                & 0.00                 \\ \hline
\multicolumn{3}{|c|}{\textbf{Indoor}}                            \\ \hline
No. Min. Return     & No. Max. Return     & No. Plane Fitting    \\ \hline
76.44               & 1.12                & 0.00                 \\ \hline
No. Boundary Points & No. Pose Estimation & No. Decoding Failure \\ \hline
8.14                & 1.80                & 1.16                 \\ \hline
\multicolumn{3}{|c|}{\textbf{Indoor Cartographer Dataset}}       \\ \hline
No. Min. Return     & No. Max. Return     & No. Plane Fitting    \\ \hline
65.76               & 0                   & 1.90                 \\ \hline
No. Boundary Points & No. Pose Estimation & No. Decoding Failure \\ \hline
0.35                & 0                   & 0                    \\ \hline
\multicolumn{3}{|c|}{\textbf{Outdoor H3D Dataset}}               \\ \hline
No. Min. Return     & No. Max. Return     & No. Plane Fitting    \\ \hline
713.35              & 8.72                & 44.41                \\ \hline
No. Boundary Points & No. Pose Estimation & No. Decoding Failure \\ \hline
2.74                & 0.38                & 0                    \\ \hline
\end{tabular}
}
\end{table}


\begin{table}[t]
\center
\caption{
    The original double sum in \eqref{eq:InnerProduct} is too slow to achieve a
    real-time application. This table compares different methods to compute the
    double sum, in which the TBB stands for Threading Building Blocks library from
Intel. Additionally, we also apply a k-d tree data structure to speed up the querying
process; the k-d tree, however, does not produce fast enough results. The unit in
the table is milliseconds.
}
\label{tab:decodingMethods}
\resizebox{0.85\columnwidth}{!}{%
\begin{tabular}{|c|c|c|}
\hline
Original Double Sum & Matrix Form     & Vector From \\ \hline
144.18              & 67.11           & 8.51        \\ \hline
TBB Original Form   & TBB Vector Form & TBB k-d tree \\ \hline
35.68               & 2.40            & 5.73        \\ \hline
\end{tabular}
}
\end{table}




\begin{table}[t]
\center
\caption{
    This table shows the numbers of false positive rejection of the proposed algorithm.
    We validated the rejection rate on the indoor Google Cartographer dataset and
    the outdoor Honda H3D datasets. The former has two VLP-16 Velodyne \lidar and the
latter has one 64-beam Velodyne \lidarN.
}
\label{tab:falsePositives}
\resizebox{0.9\columnwidth}{!}{%
\begin{tabular}{|c|c|c|}
\hline
                    & Google Cartographer & Honda H3D             \\ \hline
Scene               & Indoor Museum       & Crowed Driving Scenes \\ \hline
Duration            & 150 minutes         & 48 minutes               \\ \hline
No. Scans           & 350 thousand       & 29 thousand             \\ \hline
No. False Positives & 0                   & 0                     \\ \hline
\end{tabular}
}
\end{table}

